Stellar Populations in the Transition Region of Nuclear Star Cluster and Nuclear Stellar Disc

The Milky Way nuclear star cluster (NSC) is located within the nuclear stellar disc (NSD) in the Galactic centre. It is not fully understood if the formation and evolution of these two components are connected, and how they influence each other. We study the stellar populations in the transition region of NSC and NSD. We observed two $\sim$4.3 pc$^2$ fields with the integral-field spectrograph KMOS (VLT), located at r$\sim$20 pc (> 4 R$_e$) to the Galactic East and West of the NSC. We extract and analyse medium-resolution stellar spectra of >200 stars per field. The data contain in total nine young star candidates. We use stellar photometry to estimate the stellar masses, effective temperatures, and spectral types of the young stars. The stars are consistent with an age of 4-6 Myr, they may have formed inside the Quintuplet cluster, but were dispersed in dynamical interactions. Most stars in the two fields are red giant stars, and we measure their stellar metallicities [M/H] using full spectral fitting. We compare our [M/H] distributions to the NSC and NSD, using data from the literature, and find that the overall metallicity decreases from the central NSC, over the transition region, to the NSD. The steep decrease of [M/H] from the NSC to the region dominated by the NSD indicates that the two components have distinct stellar populations and formation histories.

==> table_parameter_nesw.tex <==
\begin{table}
\caption{Stellar parameters: Stellar identification number Id, the coordinates in R.A. and Dec, the stellar parameters $\teff$, $\mh$, $\logg$, $v_z$, and extinction corrected $K_S$-band magnitude $K_{S,0}$. }
\label{tab:parameter}
\begin{tabular}{cccccccccccccccc}
Id & R.A.& Dec & $\teff$ & $\sigma_{\teff}$ & $\mh$&$\sigma_{\mh}$ & $\logg$&$\sigma_{\logg}$ & $v_z$& $K_{S,0}$\\
&$ \left( ^{\circ} \right)$&$ \left( ^{\circ} \right)$&$ \left( \mathrm{K} \right)$&$ \left( \mathrm{K} \right)$&$ \left( \mathrm{dex} \right)$&$ \left[ \mathrm{dex} \right]$&$ \left( \mathrm{dex} \right)$&$ \left( \mathrm{dex} \right)$&$\left( \mathrm{km}\,\mathrm{s}^{-1} \right)$&$\left( \mathrm{mag} \right)$&\\
\hline
$ 900013$&$  266.50064 $&$   -28.891012 $&$  3560 $&$ ^{+360}_{-360} $&$  0.06 $&$ ^{+0.40}_{-0.40} $&$  0.3 $&$ ^{+1.1}_{-1.1} $&$     -9.4 $&$ ^{+ 3.6}_{- 3.6} $&$   8.55 $ \\
$ 900015$&$  266.50885 $&$   -28.877468 $&$  3960 $&$ ^{+270}_{-270} $&$ -0.14 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     68.8 $&$ ^{+ 1.8}_{- 1.8} $&$  10.12 $ \\
$ 900018$&$  266.50937 $&$   -28.878529 $&$  3440 $&$ ^{+270}_{-270} $&$  0.32 $&$ ^{+0.37}_{-0.37} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     64.3 $&$ ^{+ 6.9}_{- 6.9} $&$   8.77 $ \\
$ 900019$&$  266.50790 $&$   -28.879641 $&$  3650 $&$ ^{+280}_{-280} $&$  0.33 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     49.8 $&$ ^{+ 0.4}_{- 0.4} $&$  10.30 $ \\
$ 900020$&$  266.50800 $&$   -28.878771 $&$  3820 $&$ ^{+320}_{-320} $&$ -0.15 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    135.4 $&$ ^{+ 1.9}_{- 1.9} $&$  10.76 $ \\
$ 900025$&$  266.50781 $&$   -28.881580 $&$  3830 $&$ ^{+270}_{-280} $&$  0.22 $&$ ^{+0.33}_{-0.33} $&$  0.5 $&$ ^{+1.1}_{-1.1} $&$     22.0 $&$ ^{+ 1.1}_{- 1.1} $&$  10.56 $ \\
$ 900026$&$  266.51166 $&$   -28.877937 $&$  3600 $&$ ^{+270}_{-270} $&$  0.33 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    108.1 $&$ ^{+ 1.3}_{- 1.3} $&$  10.44 $ \\
$ 900029$&$  266.51059 $&$   -28.877153 $&$  3310 $&$ ^{+280}_{-280} $&$  0.44 $&$ ^{+0.39}_{-0.39} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     24.3 $&$ ^{+ 4.1}_{- 4.1} $&$   9.13 $ \\
$ 900030$&$  266.50827 $&$   -28.879345 $&$  4270 $&$ ^{+320}_{-320} $&$ -0.14 $&$ ^{+0.53}_{-0.53} $&$  0.7 $&$ ^{+1.4}_{-1.4} $&$   -155.1 $&$ ^{+ 5.5}_{- 5.5} $&$  11.27 $ \\
$ 900033$&$  266.50665 $&$   -28.881577 $&$  3630 $&$ ^{+280}_{-280} $&$  0.32 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     -8.5 $&$ ^{+ 3.1}_{- 3.1} $&$  10.95 $ \\
$ 900035$&$  266.50974 $&$   -28.879183 $&$  3760 $&$ ^{+280}_{-280} $&$  0.03 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -36.0 $&$ ^{+ 5.2}_{- 5.2} $&$  11.28 $ \\
$ 900038$&$  266.51154 $&$   -28.875957 $&$  4310 $&$ ^{+280}_{-280} $&$ -0.06 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     92.2 $&$ ^{+ 3.1}_{- 3.1} $&$  11.75 $ \\
$ 900041$&$  266.50436 $&$   -28.886799 $&$  3690 $&$ ^{+330}_{-330} $&$ -0.08 $&$ ^{+0.53}_{-0.53} $&$  0.3 $&$ ^{+1.1}_{-1.1} $&$     54.3 $&$ ^{+ 4.2}_{- 4.2} $&$  10.09 $ \\
$ 900042$&$  266.50491 $&$   -28.883879 $&$  3560 $&$ ^{+290}_{-290} $&$  0.34 $&$ ^{+0.37}_{-0.37} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     83.5 $&$ ^{+ 2.5}_{- 2.5} $&$  10.69 $ \\
$ 900043$&$  266.50940 $&$   -28.877110 $&$  4400 $&$ ^{+290}_{-290} $&$ -0.44 $&$ ^{+0.35}_{-0.35} $&$  3.6 $&$ ^{+1.1}_{-1.0} $&$    -11.2 $&$ ^{+ 3.4}_{- 3.1} $&$  11.80 $ \\
$ 900044$&$  266.50491 $&$   -28.884699 $&$  3660 $&$ ^{+280}_{-280} $&$  0.28 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    141.4 $&$ ^{+ 0.6}_{- 0.6} $&$  10.72 $ \\
$ 900046$&$  266.51089 $&$   -28.877007 $&$  3710 $&$ ^{+510}_{-510} $&$  0.40 $&$ ^{+0.35}_{-0.35} $&$  0.4 $&$ ^{+1.1}_{-1.1} $&$     -4.0 $&$ ^{+ 9.0}_{- 9.0} $&$  11.88 $ \\
$ 900047$&$  266.50696 $&$   -28.884068 $&$  3820 $&$ ^{+270}_{-270} $&$  0.10 $&$ ^{+0.40}_{-0.40} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     24.4 $&$ ^{+ 3.9}_{- 3.9} $&$  11.13 $ \\
$ 900049$&$  266.50284 $&$   -28.890535 $&$  3420 $&$ ^{+280}_{-280} $&$  0.12 $&$ ^{+0.35}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.0} $&$    104.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.58 $ \\
$ 900050$&$  266.51025 $&$   -28.875927 $&$  4090 $&$ ^{+290}_{-290} $&$  0.44 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$     86.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.21 $ \\
$ 900052$&$  266.50964 $&$   -28.877506 $&$  3870 $&$ ^{+280}_{-280} $&$  0.09 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$      3.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.72 $ \\
$ 900053$&$  266.50937 $&$   -28.876892 $&$  3780 $&$ ^{+290}_{-290} $&$  0.07 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    179.4 $&$ ^{+ 3.1}_{- 3.1} $&$  11.66 $ \\
$ 900059$&$  266.50986 $&$   -28.878139 $&$  3930 $&$ ^{+280}_{-280} $&$  0.18 $&$ ^{+0.37}_{-0.37} $&$  0.8 $&$ ^{+1.3}_{-1.3} $&$    -98.0 $&$ ^{+ 8.5}_{- 8.5} $&$  11.96 $ \\
$ 900062$&$  266.50531 $&$   -28.884296 $&$  3890 $&$ ^{+270}_{-270} $&$  0.20 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     -9.1 $&$ ^{+ 0.7}_{- 0.6} $&$  11.42 $ \\
$ 900063$&$  266.50439 $&$   -28.886585 $&$  3720 $&$ ^{+280}_{-300} $&$ -0.33 $&$ ^{+0.33}_{-0.33} $&$  0.4 $&$ ^{+1.1}_{-1.1} $&$   -139.2 $&$ ^{+ 3.1}_{- 3.1} $&$  10.90 $ \\
$ 900064$&$  266.50266 $&$   -28.888597 $&$  4810 $&$ ^{+310}_{-310} $&$ -0.59 $&$ ^{+0.36}_{-0.35} $&$  3.9 $&$ ^{+1.3}_{-1.1} $&$    140.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.13 $ \\
$ 900065$&$  266.50433 $&$   -28.884972 $&$  3850 $&$ ^{+280}_{-280} $&$  0.05 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -94.9 $&$ ^{+ 1.1}_{- 1.1} $&$  11.35 $ \\
$ 900066$&$  266.50549 $&$   -28.885521 $&$  3960 $&$ ^{+290}_{-290} $&$ -0.07 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     40.4 $&$ ^{+ 5.4}_{- 5.4} $&$  11.37 $ \\
$ 900067$&$  266.50186 $&$   -28.889297 $&$  3990 $&$ ^{+280}_{-280} $&$  0.86 $&$ ^{+0.35}_{-0.35} $&$  2.8 $&$ ^{+1.0}_{-1.0} $&$     92.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.21 $ \\
$ 900070$&$  266.50266 $&$   -28.886463 $&$  3870 $&$ ^{+280}_{-280} $&$  0.14 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     82.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.69 $ \\
$ 900073$&$  266.50739 $&$   -28.881273 $&$  4220 $&$ ^{+290}_{-290} $&$  0.25 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     57.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.38 $ \\
$ 900075$&$  266.51047 $&$   -28.877871 $&$  5050 $&$ ^{+300}_{-300} $&$ -0.34 $&$ ^{+0.39}_{-0.38} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$    -76.0 $&$ ^{+ 8.4}_{- 9.9} $&$  12.59 $ \\
$ 900076$&$  266.50574 $&$   -28.883980 $&$  3930 $&$ ^{+270}_{-270} $&$ -0.19 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     56.5 $&$ ^{+ 0.7}_{- 0.7} $&$  11.59 $ \\
$ 900085$&$  266.51065 $&$   -28.876657 $&$  4000 $&$ ^{+280}_{-300} $&$  0.45 $&$ ^{+0.35}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$      4.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.79 $ \\
$ 900087$&$  266.50421 $&$   -28.887079 $&$  3770 $&$ ^{+290}_{-280} $&$  0.88 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     34.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.11 $ \\
$ 900090$&$  266.50314 $&$   -28.887152 $&$  4270 $&$ ^{+320}_{-320} $&$  0.47 $&$ ^{+0.41}_{-0.41} $&$  3.1 $&$ ^{+1.3}_{-1.3} $&$     30.7 $&$ ^{+ 3.5}_{- 3.5} $&$  12.05 $ \\
$ 900098$&$  266.50589 $&$   -28.885382 $&$  3760 $&$ ^{+290}_{-290} $&$  0.22 $&$ ^{+0.33}_{-0.33} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$     81.0 $&$ ^{+ 1.5}_{- 1.4} $&$  11.78 $ \\
$ 900109$&$  266.50537 $&$   -28.885698 $&$  3970 $&$ ^{+290}_{-290} $&$  0.47 $&$ ^{+0.41}_{-0.41} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     30.5 $&$ ^{+ 3.8}_{- 3.8} $&$  12.15 $ \\
$ 900113$&$  266.51004 $&$   -28.876379 $&$  4190 $&$ ^{+290}_{-290} $&$  0.12 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     16.1 $&$ ^{+ 3.1}_{- 3.1} $&$  13.02 $ \\
$ 900114$&$  266.51093 $&$   -28.877487 $&$  4120 $&$ ^{+270}_{-280} $&$  0.46 $&$ ^{+0.66}_{-0.66} $&$  1.9 $&$ ^{+2.8}_{-2.8} $&$     92.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.99 $ \\
$ 900127$&$  266.51141 $&$   -28.877996 $&$  3700 $&$ ^{+280}_{-280} $&$  0.84 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    108.9 $&$ ^{+ 3.5}_{- 3.4} $&$  12.89 $ \\
$ 900130$&$  266.50842 $&$   -28.880890 $&$  3910 $&$ ^{+280}_{-280} $&$  0.31 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     91.7 $&$ ^{+ 3.8}_{- 3.9} $&$  12.91 $ \\
$ 900134$&$  266.50778 $&$   -28.880566 $&$  4680 $&$ ^{+310}_{-300} $&$ -0.09 $&$ ^{+0.36}_{-0.34} $&$  4.2 $&$ ^{+1.1}_{-1.0} $&$     -0.1 $&$ ^{+ 3.7}_{- 4.0} $&$  13.10 $ \\
$ 900146$&$  266.50952 $&$   -28.879192 $&$  3830 $&$ ^{+280}_{-280} $&$  0.60 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -33.8 $&$ ^{+ 3.1}_{- 3.1} $&$  13.34 $ \\
$ 900150$&$  266.51163 $&$   -28.877602 $&$  3660 $&$ ^{+280}_{-290} $&$  0.31 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -18.4 $&$ ^{+ 3.1}_{- 3.1} $&$  11.99 $ \\
$ 900153$&$  266.50604 $&$   -28.883083 $&$  4010 $&$ ^{+280}_{-280} $&$  0.65 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     62.0 $&$ ^{+ 3.1}_{- 3.1} $&$  13.05 $ \\
$ 900156$&$  266.50873 $&$   -28.879292 $&$  3980 $&$ ^{+320}_{-310} $&$  0.74 $&$ ^{+0.35}_{-0.36} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$     11.3 $&$ ^{+ 3.6}_{- 3.3} $&$  13.13 $ \\
$ 900173$&$  266.50391 $&$   -28.878881 $&$  3720 $&$ ^{+350}_{-350} $&$ -0.45 $&$ ^{+0.38}_{-0.38} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$   -137.6 $&$ ^{+ 1.5}_{- 1.5} $&$   8.17 $ \\
$ 900175$&$  266.49762 $&$   -28.880814 $&$  4550 $&$ ^{+280}_{-280} $&$ -1.50 $&$ ^{+0.35}_{-0.35} $&$  4.0 $&$ ^{+1.0}_{-1.0} $&$    131.6 $&$ ^{+ 9.8}_{- 9.2} $&$   8.75 $ \\
$ 900176$&$  266.50412 $&$   -28.873419 $&$  3380 $&$ ^{+310}_{-310} $&$ -0.09 $&$ ^{+0.47}_{-0.47} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    240.0 $&$ ^{+ 4.9}_{- 4.9} $&$   8.12 $ \\
$ 900178$&$  266.50229 $&$   -28.877493 $&$  3440 $&$ ^{+270}_{-270} $&$  0.32 $&$ ^{+0.33}_{-0.33} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     75.1 $&$ ^{+ 3.4}_{- 3.4} $&$   8.25 $ \\
$ 900180$&$  266.50766 $&$   -28.876329 $&$  3680 $&$ ^{+280}_{-280} $&$ -1.20 $&$ ^{+0.38}_{-0.38} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$   -106.5 $&$ ^{+ 6.3}_{- 6.3} $&$   8.88 $ \\
$ 900182$&$  266.50586 $&$   -28.880190 $&$  3510 $&$ ^{+280}_{-280} $&$ -0.36 $&$ ^{+0.37}_{-0.37} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     48.2 $&$ ^{+ 5.3}_{- 5.3} $&$   8.50 $ \\
$ 900187$&$  266.49615 $&$   -28.879761 $&$  3600 $&$ ^{+280}_{-280} $&$  0.13 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     73.4 $&$ ^{+ 3.1}_{- 3.1} $&$   8.49 $ \\
$ 900188$&$  266.49991 $&$   -28.874348 $&$  3380 $&$ ^{+280}_{-280} $&$  0.28 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -31.3 $&$ ^{+ 5.3}_{- 5.3} $&$   8.22 $ \\
$ 900192$&$  266.50394 $&$   -28.874496 $&$  3630 $&$ ^{+280}_{-280} $&$ -0.01 $&$ ^{+0.39}_{-0.39} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     22.0 $&$ ^{+ 6.8}_{- 6.8} $&$   8.95 $ \\
$ 900197$&$  266.50461 $&$   -28.874992 $&$  3450 $&$ ^{+270}_{-270} $&$  0.32 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -85.3 $&$ ^{+ 5.8}_{- 5.8} $&$   9.41 $ \\
$ 900198$&$  266.49402 $&$   -28.887918 $&$  3910 $&$ ^{+280}_{-280} $&$ -0.57 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     74.0 $&$ ^{+ 3.1}_{- 3.1} $&$   9.73 $ \\
$ 900201$&$  266.49402 $&$   -28.883238 $&$  3710 $&$ ^{+280}_{-280} $&$  0.09 $&$ ^{+0.35}_{-0.35} $&$  0.6 $&$ ^{+1.0}_{-1.0} $&$    -14.6 $&$ ^{+ 3.1}_{- 3.1} $&$   9.41 $ \\
$ 900203$&$  266.50281 $&$   -28.876125 $&$  3690 $&$ ^{+330}_{-330} $&$ -0.35 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    200.0 $&$ ^{+ 2.8}_{- 2.8} $&$   9.71 $ \\
$ 900205$&$  266.49551 $&$   -28.885778 $&$  3420 $&$ ^{+280}_{-280} $&$  0.43 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     49.3 $&$ ^{+ 3.1}_{- 3.1} $&$   9.43 $ \\
$ 900206$&$  266.49448 $&$   -28.884207 $&$  3570 $&$ ^{+280}_{-280} $&$ -0.16 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     92.8 $&$ ^{+ 3.4}_{- 3.4} $&$   9.19 $ \\
$ 900208$&$  266.50027 $&$   -28.886377 $&$  3850 $&$ ^{+290}_{-290} $&$ -0.17 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -229.4 $&$ ^{+ 5.0}_{- 5.0} $&$  10.08 $ \\
$ 900209$&$  266.49100 $&$   -28.885147 $&$  3430 $&$ ^{+280}_{-280} $&$  0.37 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     40.8 $&$ ^{+ 3.1}_{- 3.1} $&$   9.58 $ \\
$ 900210$&$  266.50098 $&$   -28.885124 $&$  3650 $&$ ^{+280}_{-280} $&$  0.18 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     76.8 $&$ ^{+ 4.3}_{- 4.3} $&$   9.64 $ \\
$ 900212$&$  266.49500 $&$   -28.881924 $&$  3660 $&$ ^{+280}_{-280} $&$  0.09 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$      4.1 $&$ ^{+ 3.1}_{- 3.1} $&$   9.86 $ \\
$ 900216$&$  266.50034 $&$   -28.877588 $&$  3820 $&$ ^{+330}_{-330} $&$ -0.15 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     33.5 $&$ ^{+ 6.7}_{- 6.7} $&$   9.74 $ \\
$ 900217$&$  266.50513 $&$   -28.876862 $&$  3790 $&$ ^{+300}_{-300} $&$  0.11 $&$ ^{+0.33}_{-0.33} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     36.0 $&$ ^{+ 0.7}_{- 0.7} $&$   9.42 $ \\
$ 900220$&$  266.49771 $&$   -28.878067 $&$  3570 $&$ ^{+330}_{-330} $&$  0.29 $&$ ^{+0.33}_{-0.33} $&$  0.4 $&$ ^{+1.1}_{-1.1} $&$     69.9 $&$ ^{+ 5.5}_{- 5.5} $&$   9.69 $ \\
$ 900223$&$  266.50623 $&$   -28.876276 $&$  3670 $&$ ^{+340}_{-340} $&$  0.21 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -119.8 $&$ ^{+ 3.6}_{- 3.6} $&$  10.51 $ \\
$ 900228$&$  266.50412 $&$   -28.878735 $&$  3810 $&$ ^{+280}_{-280} $&$ -0.28 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    176.7 $&$ ^{+ 3.6}_{- 3.6} $&$  10.19 $ \\
$ 900229$&$  266.49963 $&$   -28.887005 $&$  3510 $&$ ^{+290}_{-290} $&$  0.37 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     48.0 $&$ ^{+ 3.8}_{- 3.8} $&$  10.09 $ \\
$ 900230$&$  266.49353 $&$   -28.884953 $&$  3470 $&$ ^{+270}_{-270} $&$  0.22 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$      5.7 $&$ ^{+ 4.4}_{- 4.4} $&$   9.31 $ \\
$ 900231$&$  266.50598 $&$   -28.874863 $&$  3810 $&$ ^{+290}_{-290} $&$  0.13 $&$ ^{+0.33}_{-0.33} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     35.3 $&$ ^{+ 0.8}_{- 0.8} $&$  10.49 $ \\
$ 900232$&$  266.50375 $&$   -28.882980 $&$  3420 $&$ ^{+270}_{-270} $&$  0.39 $&$ ^{+0.34}_{-0.34} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     57.3 $&$ ^{+ 1.7}_{- 1.7} $&$   9.38 $ \\
$ 900233$&$  266.50427 $&$   -28.874014 $&$  3870 $&$ ^{+280}_{-280} $&$  0.05 $&$ ^{+0.33}_{-0.33} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     29.1 $&$ ^{+ 0.5}_{- 0.5} $&$  10.41 $ \\
$ 900236$&$  266.49792 $&$   -28.886999 $&$  3850 $&$ ^{+290}_{-290} $&$ -0.06 $&$ ^{+0.38}_{-0.38} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     64.2 $&$ ^{+ 3.4}_{- 3.4} $&$  10.66 $ \\
$ 900240$&$  266.49222 $&$   -28.887465 $&$  3610 $&$ ^{+280}_{-280} $&$  0.48 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -89.3 $&$ ^{+ 3.1}_{- 3.1} $&$   9.97 $ \\
$ 900242$&$  266.50253 $&$   -28.873726 $&$  4220 $&$ ^{+280}_{-280} $&$ -0.37 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -80.6 $&$ ^{+ 5.1}_{- 5.1} $&$  10.72 $ \\
$ 900247$&$  266.50092 $&$   -28.880808 $&$  3580 $&$ ^{+270}_{-270} $&$  0.30 $&$ ^{+0.34}_{-0.34} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     69.6 $&$ ^{+ 4.0}_{- 4.0} $&$  10.08 $ \\
$ 900249$&$  266.49863 $&$   -28.876444 $&$  3480 $&$ ^{+280}_{-280} $&$  0.43 $&$ ^{+0.35}_{-0.35} $&$  0.4 $&$ ^{+1.1}_{-1.1} $&$    -34.0 $&$ ^{+ 1.3}_{- 1.3} $&$  10.34 $ \\
$ 900256$&$  266.50446 $&$   -28.883268 $&$  2950 $&$ ^{+270}_{-270} $&$  0.33 $&$ ^{+0.66}_{-0.66} $&$  0.6 $&$ ^{+1.2}_{-1.2} $&$     86.4 $&$ ^{+ 1.1}_{- 1.1} $&$   8.57 $ \\
$ 900257$&$  266.49716 $&$   -28.886787 $&$  3720 $&$ ^{+300}_{-300} $&$  0.08 $&$ ^{+0.53}_{-0.53} $&$  0.4 $&$ ^{+1.1}_{-1.1} $&$     71.9 $&$ ^{+ 4.8}_{- 4.8} $&$  10.63 $ \\
$ 900259$&$  266.49408 $&$   -28.887028 $&$  4630 $&$ ^{+280}_{-300} $&$ -0.55 $&$ ^{+0.35}_{-0.35} $&$  3.5 $&$ ^{+1.1}_{-1.0} $&$     60.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.37 $ \\
$ 900260$&$  266.49664 $&$   -28.889442 $&$  3840 $&$ ^{+280}_{-280} $&$  0.32 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     19.4 $&$ ^{+ 3.1}_{- 3.1} $&$  10.77 $ \\
$ 900263$&$  266.50650 $&$   -28.876738 $&$  3870 $&$ ^{+270}_{-270} $&$  0.12 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     16.7 $&$ ^{+ 1.5}_{- 1.5} $&$  10.38 $ \\
$ 900264$&$  266.50574 $&$   -28.877592 $&$  3720 $&$ ^{+270}_{-270} $&$ -0.11 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    144.2 $&$ ^{+ 4.2}_{- 4.2} $&$  10.75 $ \\
$ 900266$&$  266.49963 $&$   -28.873295 $&$  3860 $&$ ^{+270}_{-270} $&$  0.25 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -35.1 $&$ ^{+ 5.8}_{- 5.8} $&$  10.56 $ \\
$ 900267$&$  266.50479 $&$   -28.872326 $&$  3820 $&$ ^{+290}_{-280} $&$  0.36 $&$ ^{+0.35}_{-0.37} $&$  0.3 $&$ ^{+1.0}_{-1.1} $&$    122.8 $&$ ^{+ 3.1}_{- 3.1} $&$  10.72 $ \\
$ 900272$&$  266.49799 $&$   -28.888784 $&$  3970 $&$ ^{+280}_{-280} $&$ -0.26 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     89.9 $&$ ^{+ 3.1}_{- 3.1} $&$  10.93 $ \\
$ 900274$&$  266.50497 $&$   -28.872589 $&$  3610 $&$ ^{+280}_{-280} $&$  0.29 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     53.8 $&$ ^{+ 3.1}_{- 3.1} $&$  10.31 $ \\
$ 900276$&$  266.50027 $&$   -28.885855 $&$  3800 $&$ ^{+280}_{-280} $&$  0.03 $&$ ^{+0.48}_{-0.48} $&$  0.4 $&$ ^{+1.1}_{-1.1} $&$    131.4 $&$ ^{+ 1.0}_{- 1.0} $&$  10.94 $ \\
$ 900278$&$  266.49866 $&$   -28.880999 $&$  3870 $&$ ^{+280}_{-280} $&$ -0.16 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    330.5 $&$ ^{+ 3.1}_{- 3.1} $&$  10.26 $ \\
$ 900282$&$  266.50085 $&$   -28.874977 $&$  3610 $&$ ^{+300}_{-300} $&$  0.74 $&$ ^{+0.36}_{-0.36} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     42.9 $&$ ^{+ 2.2}_{- 2.2} $&$  10.85 $ \\
$ 900286$&$  266.49918 $&$   -28.878345 $&$  3830 $&$ ^{+280}_{-280} $&$  0.08 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    130.6 $&$ ^{+ 2.2}_{- 2.2} $&$  11.02 $ \\
$ 900288$&$  266.49582 $&$   -28.880859 $&$  3770 $&$ ^{+330}_{-330} $&$  0.15 $&$ ^{+0.40}_{-0.40} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -12.5 $&$ ^{+ 4.3}_{- 4.3} $&$  11.37 $ \\
$ 900289$&$  266.50443 $&$   -28.879034 $&$  3820 $&$ ^{+280}_{-280} $&$  0.06 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -25.9 $&$ ^{+ 4.5}_{- 4.5} $&$  10.71 $ \\
$ 900292$&$  266.50287 $&$   -28.880507 $&$  3880 $&$ ^{+280}_{-280} $&$  0.13 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -79.3 $&$ ^{+ 3.1}_{- 3.1} $&$  10.64 $ \\
$ 900296$&$  266.50769 $&$   -28.874865 $&$  3910 $&$ ^{+270}_{-270} $&$ -0.12 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     50.0 $&$ ^{+ 6.5}_{- 6.5} $&$  11.27 $ \\
$ 900297$&$  266.49854 $&$   -28.886272 $&$  3420 $&$ ^{+290}_{-290} $&$  0.43 $&$ ^{+0.33}_{-0.33} $&$  0.3 $&$ ^{+1.1}_{-1.1} $&$    -66.6 $&$ ^{+ 1.0}_{- 1.0} $&$   9.25 $ \\
$ 900298$&$  266.50848 $&$   -28.878036 $&$  3800 $&$ ^{+300}_{-300} $&$  0.24 $&$ ^{+0.38}_{-0.38} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -52.5 $&$ ^{+ 1.5}_{- 1.5} $&$  11.24 $ \\
$ 900302$&$  266.49368 $&$   -28.885681 $&$  4190 $&$ ^{+280}_{-280} $&$ -0.19 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     39.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.07 $ \\
$ 900303$&$  266.50546 $&$   -28.873281 $&$  3440 $&$ ^{+280}_{-280} $&$  0.18 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     68.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.26 $ \\
$ 900304$&$  266.49146 $&$   -28.884560 $&$  3870 $&$ ^{+280}_{-280} $&$  0.22 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     41.6 $&$ ^{+ 3.1}_{- 3.1} $&$  11.26 $ \\
$ 900305$&$  266.49768 $&$   -28.886808 $&$  3890 $&$ ^{+280}_{-280} $&$  0.04 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     25.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.32 $ \\
$ 900306$&$  266.50653 $&$   -28.874632 $&$  3860 $&$ ^{+280}_{-270} $&$  0.20 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     38.5 $&$ ^{+ 0.7}_{- 0.7} $&$  11.18 $ \\
$ 900309$&$  266.50479 $&$   -28.874516 $&$  3580 $&$ ^{+280}_{-270} $&$  0.52 $&$ ^{+0.32}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     -4.4 $&$ ^{+ 2.8}_{- 2.8} $&$  11.42 $ \\
$ 900311$&$  266.49969 $&$   -28.883242 $&$  4380 $&$ ^{+280}_{-280} $&$  0.05 $&$ ^{+0.35}_{-0.35} $&$  0.3 $&$ ^{+1.0}_{-1.1} $&$   -199.9 $&$ ^{+ 3.1}_{- 3.1} $&$  11.29 $ \\
$ 900312$&$  266.50000 $&$   -28.887081 $&$  3760 $&$ ^{+300}_{-300} $&$  0.36 $&$ ^{+0.43}_{-0.43} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$      4.0 $&$ ^{+ 6.4}_{- 6.4} $&$  11.20 $ \\
$ 900318$&$  266.50604 $&$   -28.879103 $&$  4090 $&$ ^{+310}_{-310} $&$ -0.23 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     13.3 $&$ ^{+ 0.9}_{- 0.9} $&$  11.15 $ \\
$ 900319$&$  266.50879 $&$   -28.876755 $&$  3900 $&$ ^{+270}_{-270} $&$  0.00 $&$ ^{+0.46}_{-0.46} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    132.5 $&$ ^{+ 1.6}_{- 1.6} $&$  11.78 $ \\
$ 900320$&$  266.50208 $&$   -28.886627 $&$  3730 $&$ ^{+390}_{-390} $&$  0.40 $&$ ^{+0.34}_{-0.34} $&$  0.4 $&$ ^{+1.1}_{-1.1} $&$    -29.7 $&$ ^{+ 2.5}_{- 2.5} $&$  10.89 $ \\
$ 900323$&$  266.50824 $&$   -28.877251 $&$  4050 $&$ ^{+310}_{-310} $&$ -0.08 $&$ ^{+0.41}_{-0.41} $&$  0.4 $&$ ^{+1.0}_{-1.0} $&$    -30.8 $&$ ^{+ 4.5}_{- 4.5} $&$  11.77 $ \\
$ 900325$&$  266.49341 $&$   -28.885668 $&$  4050 $&$ ^{+280}_{-280} $&$ -0.16 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     55.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.42 $ \\
$ 900329$&$  266.50424 $&$   -28.877331 $&$  3500 $&$ ^{+280}_{-280} $&$  0.55 $&$ ^{+0.37}_{-0.37} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -76.2 $&$ ^{+ 7.1}_{- 7.1} $&$  11.04 $ \\
$ 900335$&$  266.50955 $&$   -28.875790 $&$  3850 $&$ ^{+320}_{-270} $&$  0.19 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     31.5 $&$ ^{+ 3.1}_{- 3.1} $&$  11.60 $ \\
$ 900337$&$  266.50616 $&$   -28.874592 $&$  3490 $&$ ^{+290}_{-290} $&$  0.30 $&$ ^{+0.34}_{-0.34} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     92.1 $&$ ^{+ 3.7}_{- 3.7} $&$  10.29 $ \\
$ 900338$&$  266.50433 $&$   -28.874512 $&$  3750 $&$ ^{+330}_{-330} $&$  0.15 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -35.4 $&$ ^{+ 3.3}_{- 3.3} $&$  11.34 $ \\
$ 900340$&$  266.50034 $&$   -28.875010 $&$  3640 $&$ ^{+290}_{-290} $&$  0.15 $&$ ^{+0.37}_{-0.37} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     48.7 $&$ ^{+ 1.5}_{- 1.4} $&$  11.51 $ \\
$ 900343$&$  266.49524 $&$   -28.886209 $&$  3880 $&$ ^{+270}_{-270} $&$  0.37 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     61.1 $&$ ^{+ 0.8}_{- 0.8} $&$  11.41 $ \\
$ 900347$&$  266.49557 $&$   -28.887297 $&$  4040 $&$ ^{+330}_{-330} $&$  0.09 $&$ ^{+0.41}_{-0.41} $&$  1.0 $&$ ^{+1.0}_{-1.0} $&$    132.4 $&$ ^{+ 3.3}_{- 3.3} $&$  11.84 $ \\
$ 900349$&$  266.49655 $&$   -28.887817 $&$  3940 $&$ ^{+280}_{-280} $&$ -0.12 $&$ ^{+0.36}_{-0.36} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     17.2 $&$ ^{+ 2.8}_{- 2.8} $&$  11.71 $ \\
$ 900350$&$  266.50336 $&$   -28.877386 $&$  4060 $&$ ^{+340}_{-340} $&$ -0.52 $&$ ^{+0.43}_{-0.43} $&$  0.6 $&$ ^{+1.2}_{-1.2} $&$    111.2 $&$ ^{+ 5.0}_{- 5.0} $&$  11.84 $ \\
$ 900353$&$  266.49908 $&$   -28.883139 $&$  4300 $&$ ^{+280}_{-280} $&$ -0.06 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.1} $&$     77.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.27 $ \\
$ 900354$&$  266.50107 $&$   -28.874489 $&$  3770 $&$ ^{+280}_{-290} $&$  0.51 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -28.2 $&$ ^{+ 3.1}_{- 3.1} $&$  10.96 $ \\
$ 900356$&$  266.50714 $&$   -28.875257 $&$  4140 $&$ ^{+420}_{-420} $&$  0.44 $&$ ^{+0.33}_{-0.33} $&$  2.9 $&$ ^{+1.3}_{-1.3} $&$    -27.5 $&$ ^{+ 2.3}_{- 2.3} $&$  12.04 $ \\
$ 900357$&$  266.50571 $&$   -28.878433 $&$  4100 $&$ ^{+280}_{-280} $&$ -0.48 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     -1.1 $&$ ^{+ 2.2}_{- 2.2} $&$  11.91 $ \\
$ 900362$&$  266.49969 $&$   -28.889074 $&$  3760 $&$ ^{+290}_{-290} $&$  0.21 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    102.4 $&$ ^{+ 0.8}_{- 0.8} $&$  11.23 $ \\
$ 900364$&$  266.49643 $&$   -28.886204 $&$  3680 $&$ ^{+300}_{-300} $&$  0.28 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    131.8 $&$ ^{+ 0.9}_{- 0.8} $&$  11.51 $ \\
$ 900366$&$  266.50287 $&$   -28.878098 $&$  4060 $&$ ^{+360}_{-360} $&$ -0.15 $&$ ^{+0.33}_{-0.34} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     94.0 $&$ ^{+ 1.9}_{- 1.9} $&$  11.69 $ \\
$ 900370$&$  266.50070 $&$   -28.875368 $&$  3890 $&$ ^{+280}_{-280} $&$  0.08 $&$ ^{+0.33}_{-0.34} $&$  0.4 $&$ ^{+1.0}_{-1.0} $&$     47.8 $&$ ^{+ 1.3}_{- 1.3} $&$  11.63 $ \\
$ 900371$&$  266.50040 $&$   -28.878105 $&$  3660 $&$ ^{+290}_{-290} $&$  0.50 $&$ ^{+0.43}_{-0.43} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$    100.9 $&$ ^{+ 3.9}_{- 3.9} $&$  11.47 $ \\
$ 900373$&$  266.49469 $&$   -28.888268 $&$  5100 $&$ ^{+290}_{-300} $&$ -0.09 $&$ ^{+0.36}_{-0.34} $&$  3.4 $&$ ^{+1.3}_{-1.1} $&$     36.4 $&$ ^{+ 4.5}_{- 4.4} $&$  12.32 $ \\
$ 900376$&$  266.49612 $&$   -28.880926 $&$  3920 $&$ ^{+270}_{-270} $&$  0.13 $&$ ^{+0.40}_{-0.40} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    134.2 $&$ ^{+ 2.4}_{- 2.4} $&$  11.53 $ \\
$ 900379$&$  266.50244 $&$   -28.878616 $&$  3960 $&$ ^{+270}_{-270} $&$ -0.31 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    143.5 $&$ ^{+ 2.3}_{- 2.3} $&$  11.75 $ \\
$ 900380$&$  266.50018 $&$   -28.887257 $&$  3880 $&$ ^{+270}_{-270} $&$ -0.11 $&$ ^{+0.37}_{-0.37} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     49.9 $&$ ^{+ 2.3}_{- 2.3} $&$  11.74 $ \\
$ 900382$&$  266.49573 $&$   -28.881208 $&$  4130 $&$ ^{+280}_{-280} $&$ -0.08 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     78.4 $&$ ^{+ 3.1}_{- 3.1} $&$  11.97 $ \\
$ 900391$&$  266.49393 $&$   -28.885595 $&$  3910 $&$ ^{+270}_{-270} $&$  0.15 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     42.1 $&$ ^{+ 3.7}_{- 3.7} $&$  11.51 $ \\
$ 900393$&$  266.49945 $&$   -28.874586 $&$  3730 $&$ ^{+310}_{-310} $&$  0.23 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    121.0 $&$ ^{+ 2.3}_{- 2.3} $&$  11.22 $ \\
$ 900394$&$  266.50906 $&$   -28.876644 $&$  3940 $&$ ^{+280}_{-280} $&$  0.73 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    127.1 $&$ ^{+ 3.1}_{- 3.1} $&$  12.15 $ \\
$ 900398$&$  266.50479 $&$   -28.873449 $&$  4010 $&$ ^{+270}_{-290} $&$  0.72 $&$ ^{+0.36}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -35.6 $&$ ^{+ 1.1}_{- 1.1} $&$  12.03 $ \\
$ 900403$&$  266.50903 $&$   -28.875797 $&$  4260 $&$ ^{+280}_{-280} $&$ -0.21 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     73.7 $&$ ^{+ 1.3}_{- 1.3} $&$  11.98 $ \\
$ 900405$&$  266.49591 $&$   -28.886976 $&$  3830 $&$ ^{+290}_{-290} $&$  0.77 $&$ ^{+0.39}_{-0.39} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     17.8 $&$ ^{+ 1.4}_{- 1.4} $&$  12.26 $ \\
$ 900409$&$  266.49411 $&$   -28.886229 $&$  3890 $&$ ^{+270}_{-270} $&$  0.12 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     -2.0 $&$ ^{+ 0.6}_{- 0.6} $&$  11.38 $ \\
$ 900411$&$  266.49936 $&$   -28.887703 $&$  4470 $&$ ^{+280}_{-280} $&$  0.26 $&$ ^{+0.33}_{-0.33} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     31.2 $&$ ^{+ 4.4}_{- 4.4} $&$  12.04 $ \\
$ 900412$&$  266.50018 $&$   -28.873022 $&$  3890 $&$ ^{+280}_{-280} $&$  0.03 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     36.8 $&$ ^{+ 3.1}_{- 3.1} $&$  11.65 $ \\
$ 900416$&$  266.49695 $&$   -28.882545 $&$  3640 $&$ ^{+280}_{-280} $&$ -0.13 $&$ ^{+0.35}_{-0.35} $&$  0.3 $&$ ^{+1.0}_{-1.1} $&$    -20.5 $&$ ^{+ 3.1}_{- 3.1} $&$  11.41 $ \\
$ 900417$&$  266.50082 $&$   -28.872931 $&$  3860 $&$ ^{+280}_{-270} $&$  0.20 $&$ ^{+0.36}_{-0.36} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     25.4 $&$ ^{+ 4.7}_{- 4.7} $&$  11.59 $ \\
$ 900419$&$  266.50620 $&$   -28.875378 $&$  4190 $&$ ^{+290}_{-300} $&$ -0.37 $&$ ^{+0.36}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    150.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.59 $ \\
$ 900423$&$  266.49277 $&$   -28.884190 $&$  3760 $&$ ^{+280}_{-280} $&$  0.22 $&$ ^{+0.34}_{-0.34} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$    124.5 $&$ ^{+ 3.9}_{- 3.9} $&$  11.90 $ \\
$ 900424$&$  266.50174 $&$   -28.871119 $&$  3880 $&$ ^{+280}_{-280} $&$  0.27 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -63.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.87 $ \\
$ 900425$&$  266.50113 $&$   -28.878241 $&$  4380 $&$ ^{+290}_{-280} $&$  0.32 $&$ ^{+0.35}_{-0.35} $&$  2.7 $&$ ^{+1.1}_{-1.1} $&$     56.8 $&$ ^{+ 3.1}_{- 3.1} $&$  11.78 $ \\
$ 900426$&$  266.49988 $&$   -28.880966 $&$  4010 $&$ ^{+280}_{-280} $&$ -0.44 $&$ ^{+0.33}_{-0.37} $&$  0.2 $&$ ^{+1.0}_{-1.2} $&$     32.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.66 $ \\
$ 900427$&$  266.50055 $&$   -28.883507 $&$  3880 $&$ ^{+270}_{-270} $&$  0.24 $&$ ^{+0.39}_{-0.39} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     69.6 $&$ ^{+ 0.8}_{- 0.8} $&$  11.66 $ \\
$ 900429$&$  266.49829 $&$   -28.886944 $&$  3930 $&$ ^{+280}_{-280} $&$  0.20 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     91.9 $&$ ^{+ 0.9}_{- 1.0} $&$  11.79 $ \\
$ 900431$&$  266.49686 $&$   -28.877926 $&$  4060 $&$ ^{+320}_{-320} $&$ -0.09 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     44.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.48 $ \\
$ 900433$&$  266.50012 $&$   -28.882591 $&$  3680 $&$ ^{+280}_{-280} $&$  0.27 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -32.4 $&$ ^{+ 3.1}_{- 3.1} $&$  11.58 $ \\
$ 900434$&$  266.50668 $&$   -28.879446 $&$  3800 $&$ ^{+290}_{-290} $&$  0.94 $&$ ^{+0.32}_{-0.32} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     19.7 $&$ ^{+ 1.1}_{- 1.0} $&$  12.03 $ \\
$ 900436$&$  266.50031 $&$   -28.873367 $&$  3980 $&$ ^{+280}_{-280} $&$ -0.28 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     20.5 $&$ ^{+ 3.1}_{- 3.1} $&$  11.79 $ \\
$ 900440$&$  266.49716 $&$   -28.882166 $&$  4030 $&$ ^{+290}_{-280} $&$ -0.04 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     71.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.59 $ \\
$ 900443$&$  266.50110 $&$   -28.872046 $&$  4220 $&$ ^{+280}_{-280} $&$  0.25 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     82.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.02 $ \\
$ 900445$&$  266.50058 $&$   -28.888912 $&$  3950 $&$ ^{+280}_{-280} $&$  0.82 $&$ ^{+0.36}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -21.2 $&$ ^{+ 1.8}_{- 1.8} $&$  12.10 $ \\
$ 900446$&$  266.49899 $&$   -28.878466 $&$  4080 $&$ ^{+320}_{-320} $&$  0.52 $&$ ^{+0.34}_{-0.34} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     52.9 $&$ ^{+ 9.7}_{- 9.7} $&$  12.03 $ \\
$ 900447$&$  266.49243 $&$   -28.884382 $&$  3400 $&$ ^{+280}_{-280} $&$  0.52 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -194.9 $&$ ^{+ 3.1}_{- 3.1} $&$   9.94 $ \\
$ 900448$&$  266.49872 $&$   -28.881729 $&$  4060 $&$ ^{+280}_{-290} $&$ -0.18 $&$ ^{+0.36}_{-0.38} $&$  1.1 $&$ ^{+1.1}_{-1.1} $&$     20.4 $&$ ^{+ 4.8}_{- 4.3} $&$  11.67 $ \\
$ 900451$&$  266.50330 $&$   -28.882675 $&$  4120 $&$ ^{+280}_{-280} $&$ -0.03 $&$ ^{+0.34}_{-0.37} $&$  0.8 $&$ ^{+1.1}_{-1.1} $&$     64.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.46 $ \\
$ 900453$&$  266.50308 $&$   -28.884945 $&$  3880 $&$ ^{+290}_{-270} $&$  0.05 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -12.1 $&$ ^{+ 1.1}_{- 0.9} $&$  11.70 $ \\
$ 900454$&$  266.49918 $&$   -28.888824 $&$  3750 $&$ ^{+290}_{-290} $&$  0.13 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     83.5 $&$ ^{+ 2.6}_{- 2.6} $&$  11.69 $ \\
$ 900459$&$  266.50476 $&$   -28.875507 $&$  3880 $&$ ^{+280}_{-280} $&$  0.93 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    170.3 $&$ ^{+ 3.1}_{- 3.1} $&$  12.17 $ \\
$ 900462$&$  266.49866 $&$   -28.885054 $&$  4190 $&$ ^{+280}_{-300} $&$ -0.60 $&$ ^{+0.35}_{-0.35} $&$  4.3 $&$ ^{+1.1}_{-1.0} $&$    -40.4 $&$ ^{+ 3.9}_{- 3.8} $&$  12.08 $ \\
$ 900471$&$  266.50879 $&$   -28.874596 $&$  4460 $&$ ^{+310}_{-300} $&$ -0.24 $&$ ^{+0.35}_{-0.35} $&$  2.7 $&$ ^{+1.1}_{-1.1} $&$     49.3 $&$ ^{+ 4.4}_{- 4.7} $&$  12.75 $ \\
$ 900472$&$  266.49954 $&$   -28.878841 $&$  3860 $&$ ^{+280}_{-280} $&$  0.17 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -210.6 $&$ ^{+ 3.1}_{- 3.1} $&$  11.85 $ \\
$ 900473$&$  266.49762 $&$   -28.879633 $&$  4240 $&$ ^{+280}_{-280} $&$  0.23 $&$ ^{+0.37}_{-0.37} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     41.6 $&$ ^{+ 6.4}_{- 6.4} $&$  12.07 $ \\
$ 900476$&$  266.49786 $&$   -28.882978 $&$  3670 $&$ ^{+390}_{-390} $&$  0.55 $&$ ^{+0.51}_{-0.51} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -100.0 $&$ ^{+ 1.2}_{- 1.1} $&$  11.62 $ \\
$ 900478$&$  266.50250 $&$   -28.883465 $&$  3990 $&$ ^{+320}_{-320} $&$ -0.03 $&$ ^{+0.62}_{-0.62} $&$  0.6 $&$ ^{+1.1}_{-1.1} $&$     25.8 $&$ ^{+ 1.4}_{- 1.3} $&$  11.80 $ \\
$ 900479$&$  266.49945 $&$   -28.877913 $&$  4280 $&$ ^{+300}_{-290} $&$ -0.30 $&$ ^{+0.35}_{-0.35} $&$  4.2 $&$ ^{+1.0}_{-1.0} $&$     43.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.24 $ \\
$ 900480$&$  266.50375 $&$   -28.884029 $&$  4260 $&$ ^{+280}_{-280} $&$  0.02 $&$ ^{+0.34}_{-0.34} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     42.7 $&$ ^{+ 4.1}_{- 4.1} $&$  12.62 $ \\
$ 900481$&$  266.49619 $&$   -28.882257 $&$  4260 $&$ ^{+290}_{-290} $&$  0.24 $&$ ^{+0.41}_{-0.41} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$      0.9 $&$ ^{+ 6.3}_{- 6.3} $&$  12.17 $ \\
$ 900491$&$  266.49789 $&$   -28.886314 $&$  3910 $&$ ^{+280}_{-280} $&$  0.93 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     74.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.27 $ \\
$ 900493$&$  266.50610 $&$   -28.875105 $&$  4030 $&$ ^{+280}_{-280} $&$  0.47 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     26.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.48 $ \\
$ 900508$&$  266.49890 $&$   -28.880732 $&$  4370 $&$ ^{+290}_{-290} $&$ -0.05 $&$ ^{+0.35}_{-0.34} $&$  0.4 $&$ ^{+1.0}_{-1.1} $&$     44.9 $&$ ^{+ 3.4}_{- 3.3} $&$  11.79 $ \\
$ 900511$&$  266.49954 $&$   -28.881859 $&$  4100 $&$ ^{+280}_{-280} $&$  0.45 $&$ ^{+0.36}_{-0.35} $&$  2.1 $&$ ^{+1.2}_{-1.0} $&$   -324.6 $&$ ^{+ 3.1}_{- 3.1} $&$  11.83 $ \\
$ 900513$&$  266.49829 $&$   -28.883718 $&$  4100 $&$ ^{+280}_{-280} $&$  0.02 $&$ ^{+0.37}_{-0.37} $&$  2.7 $&$ ^{+1.8}_{-1.8} $&$   -236.4 $&$ ^{+ 1.7}_{- 1.7} $&$  11.98 $ \\
$ 900520$&$  266.50006 $&$   -28.875809 $&$  4280 $&$ ^{+300}_{-300} $&$  0.36 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$   -165.6 $&$ ^{+ 3.1}_{- 3.1} $&$  12.54 $ \\
$ 900521$&$  266.50360 $&$   -28.880646 $&$  3670 $&$ ^{+280}_{-280} $&$  0.63 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -60.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.99 $ \\
$ 900525$&$  266.50507 $&$   -28.881840 $&$  4380 $&$ ^{+330}_{-330} $&$  0.08 $&$ ^{+0.36}_{-0.36} $&$  3.0 $&$ ^{+1.1}_{-1.2} $&$   -192.2 $&$ ^{+ 7.6}_{- 7.2} $&$  12.45 $ \\
$ 900528$&$  266.50311 $&$   -28.882956 $&$  3820 $&$ ^{+300}_{-280} $&$  0.19 $&$ ^{+0.35}_{-0.35} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$     40.8 $&$ ^{+ 3.1}_{- 3.1} $&$  11.36 $ \\
$ 900531$&$  266.50528 $&$   -28.879442 $&$  3520 $&$ ^{+290}_{-290} $&$  0.31 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -15.7 $&$ ^{+ 3.8}_{- 3.8} $&$  11.93 $ \\
$ 900535$&$  266.50125 $&$   -28.886362 $&$  3860 $&$ ^{+280}_{-280} $&$  0.94 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     -2.1 $&$ ^{+ 3.1}_{- 3.1} $&$  12.47 $ \\
$ 900538$&$  266.50635 $&$   -28.876886 $&$  4130 $&$ ^{+280}_{-280} $&$  0.22 $&$ ^{+0.40}_{-0.40} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     22.6 $&$ ^{+ 2.1}_{- 2.1} $&$  13.19 $ \\
$ 900539$&$  266.49869 $&$   -28.876217 $&$  4690 $&$ ^{+290}_{-280} $&$ -0.15 $&$ ^{+0.35}_{-0.35} $&$  4.3 $&$ ^{+1.0}_{-1.0} $&$    109.1 $&$ ^{+ 3.1}_{- 3.1} $&$  12.09 $ \\
$ 900544$&$  266.50201 $&$   -28.872213 $&$  3950 $&$ ^{+280}_{-300} $&$  0.40 $&$ ^{+0.36}_{-0.36} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     92.1 $&$ ^{+ 3.1}_{- 3.1} $&$  12.44 $ \\
$ 900549$&$  266.50864 $&$   -28.876286 $&$  4230 $&$ ^{+320}_{-330} $&$  0.26 $&$ ^{+0.37}_{-0.36} $&$  2.7 $&$ ^{+1.1}_{-1.2} $&$     98.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.76 $ \\
$ 900553$&$  266.49957 $&$   -28.883963 $&$  4060 $&$ ^{+280}_{-280} $&$  0.73 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$    119.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.32 $ \\
$ 900554$&$  266.49933 $&$   -28.876684 $&$  3400 $&$ ^{+280}_{-280} $&$  0.31 $&$ ^{+0.42}_{-0.42} $&$  0.4 $&$ ^{+1.0}_{-1.0} $&$     14.5 $&$ ^{+ 4.8}_{- 4.8} $&$  10.38 $ \\
$ 900567$&$  266.50125 $&$   -28.875666 $&$  4130 $&$ ^{+290}_{-300} $&$  0.71 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -92.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.64 $ \\
$ 900573$&$  266.49530 $&$   -28.889109 $&$  4040 $&$ ^{+280}_{-280} $&$  0.36 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     14.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.60 $ \\
$ 900580$&$  266.50229 $&$   -28.877165 $&$  3750 $&$ ^{+310}_{-310} $&$  0.79 $&$ ^{+0.36}_{-0.36} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     53.7 $&$ ^{+13.1}_{-13.1} $&$  12.74 $ \\
$ 900582$&$  266.50082 $&$   -28.874144 $&$  3850 $&$ ^{+290}_{-280} $&$  0.61 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     25.6 $&$ ^{+ 3.1}_{- 3.1} $&$  11.82 $ \\
$ 900584$&$  266.49817 $&$   -28.883181 $&$  4760 $&$ ^{+310}_{-310} $&$  0.05 $&$ ^{+0.51}_{-0.51} $&$  3.7 $&$ ^{+1.1}_{-1.1} $&$    -64.2 $&$ ^{+ 4.4}_{- 4.8} $&$  12.70 $ \\
$ 900585$&$  266.49420 $&$   -28.887827 $&$  4280 $&$ ^{+280}_{-280} $&$ -0.77 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     68.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.90 $ \\
$ 900589$&$  266.50070 $&$   -28.872286 $&$  4510 $&$ ^{+320}_{-320} $&$  0.30 $&$ ^{+0.37}_{-0.36} $&$  3.5 $&$ ^{+1.3}_{-1.2} $&$    102.6 $&$ ^{+ 4.3}_{- 4.4} $&$  12.80 $ \\
$ 900597$&$  266.50867 $&$   -28.877546 $&$  4040 $&$ ^{+270}_{-270} $&$  0.48 $&$ ^{+0.34}_{-0.34} $&$  2.4 $&$ ^{+1.1}_{-1.1} $&$     67.6 $&$ ^{+ 2.3}_{- 2.3} $&$  12.87 $ \\
$ 900599$&$  266.49918 $&$   -28.877663 $&$  4090 $&$ ^{+280}_{-280} $&$  0.13 $&$ ^{+0.40}_{-0.40} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     89.6 $&$ ^{+ 1.4}_{- 1.5} $&$  12.08 $ \\
$ 900609$&$  266.49533 $&$   -28.880199 $&$  4480 $&$ ^{+300}_{-320} $&$  0.43 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$    -63.5 $&$ ^{+ 3.2}_{- 3.0} $&$  13.08 $ \\
$ 900612$&$  266.49780 $&$   -28.875734 $&$  3980 $&$ ^{+280}_{-280} $&$  0.95 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    116.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.08 $ \\
$ 900614$&$  266.50583 $&$   -28.876764 $&$  4250 $&$ ^{+310}_{-330} $&$ -0.12 $&$ ^{+0.38}_{-0.37} $&$  3.9 $&$ ^{+1.3}_{-1.1} $&$   -106.8 $&$ ^{+ 6.8}_{- 8.3} $&$  13.22 $ \\
$ 900618$&$  266.50342 $&$   -28.875587 $&$  3930 $&$ ^{+280}_{-280} $&$  0.92 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -34.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.47 $ \\
$ 900619$&$  266.49649 $&$   -28.879267 $&$  4130 $&$ ^{+290}_{-300} $&$  0.84 $&$ ^{+0.35}_{-0.35} $&$  3.4 $&$ ^{+1.1}_{-1.0} $&$     50.3 $&$ ^{+ 3.1}_{- 3.1} $&$  12.66 $ \\
$ 900622$&$  266.50839 $&$   -28.876711 $&$  4300 $&$ ^{+320}_{-300} $&$  0.64 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$     90.6 $&$ ^{+ 3.1}_{- 3.1} $&$  12.87 $ \\
$ 900631$&$  266.50266 $&$   -28.875185 $&$  3810 $&$ ^{+290}_{-290} $&$ -0.11 $&$ ^{+0.39}_{-0.39} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     53.7 $&$ ^{+ 1.2}_{- 1.2} $&$  11.77 $ \\
$ 900641$&$  266.50183 $&$   -28.886749 $&$  4180 $&$ ^{+300}_{-320} $&$  0.37 $&$ ^{+0.38}_{-0.35} $&$  2.6 $&$ ^{+1.1}_{-1.2} $&$     92.2 $&$ ^{+ 3.8}_{- 4.1} $&$  12.87 $ \\
$ 900644$&$  266.49481 $&$   -28.885546 $&$  4250 $&$ ^{+300}_{-300} $&$  0.26 $&$ ^{+0.34}_{-0.34} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     31.1 $&$ ^{+12.3}_{-12.3} $&$  12.55 $ \\
$ 900662$&$  266.49506 $&$   -28.884722 $&$  3940 $&$ ^{+290}_{-310} $&$  0.07 $&$ ^{+0.39}_{-0.39} $&$  0.8 $&$ ^{+1.1}_{-1.1} $&$    132.6 $&$ ^{+ 3.1}_{- 3.1} $&$  11.97 $ \\
$ 900666$&$  266.50143 $&$   -28.887306 $&$  3800 $&$ ^{+290}_{-290} $&$  0.90 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     55.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.81 $ \\
$ 900669$&$  266.50500 $&$   -28.879131 $&$  4220 $&$ ^{+320}_{-310} $&$  0.13 $&$ ^{+0.37}_{-0.38} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$     13.0 $&$ ^{+ 6.2}_{- 5.7} $&$  12.74 $ \\
$ 900676$&$  266.50104 $&$   -28.876602 $&$  4080 $&$ ^{+290}_{-330} $&$  0.58 $&$ ^{+0.35}_{-0.35} $&$  2.7 $&$ ^{+1.1}_{-1.1} $&$     86.6 $&$ ^{+ 3.1}_{- 3.1} $&$  12.91 $ \\
$ 900699$&$  266.49628 $&$   -28.887173 $&$  3860 $&$ ^{+280}_{-280} $&$  0.29 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     -5.3 $&$ ^{+ 4.5}_{- 3.6} $&$  12.98 $ \\
$ 900725$&$  266.50290 $&$   -28.882549 $&$  3950 $&$ ^{+280}_{-280} $&$  0.23 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     39.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.13 $ \\
$ 900727$&$  266.49460 $&$   -28.882822 $&$  3880 $&$ ^{+280}_{-280} $&$  0.87 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     -0.1 $&$ ^{+ 3.1}_{- 3.1} $&$  12.88 $ \\
$ 900732$&$  266.50961 $&$   -28.878115 $&$  3840 $&$ ^{+360}_{-360} $&$  0.67 $&$ ^{+0.41}_{-0.41} $&$  2.4 $&$ ^{+1.1}_{-1.1} $&$    -56.6 $&$ ^{+12.1}_{-12.1} $&$  12.46 $ \\
$ 900735$&$  266.49988 $&$   -28.884176 $&$  3940 $&$ ^{+280}_{-310} $&$  0.75 $&$ ^{+0.37}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -33.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.37 $ \\
$ 900738$&$  266.50208 $&$   -28.883825 $&$  4180 $&$ ^{+310}_{-300} $&$  0.32 $&$ ^{+0.36}_{-0.36} $&$  2.3 $&$ ^{+1.0}_{-1.2} $&$     75.7 $&$ ^{+ 4.1}_{- 3.8} $&$  12.63 $ \\
$ 900747$&$  266.50320 $&$   -28.877232 $&$  3760 $&$ ^{+270}_{-270} $&$ -0.19 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    101.9 $&$ ^{+ 1.1}_{- 1.1} $&$  11.60 $ \\
$ 900755$&$  266.49796 $&$   -28.884811 $&$  3810 $&$ ^{+300}_{-300} $&$ -0.11 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     71.3 $&$ ^{+ 1.4}_{- 1.4} $&$  11.96 $ \\
$ 900758$&$  266.49503 $&$   -28.882895 $&$  4380 $&$ ^{+280}_{-280} $&$  0.34 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     21.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.88 $ \\
$ 900824$&$  266.49915 $&$   -28.879978 $&$  4030 $&$ ^{+310}_{-310} $&$  0.32 $&$ ^{+0.62}_{-0.62} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$   -144.5 $&$ ^{+ 6.1}_{- 6.1} $&$  12.12 $ \\
$ 900826$&$  266.49713 $&$   -28.884590 $&$  4400 $&$ ^{+300}_{-290} $&$  0.44 $&$ ^{+0.35}_{-0.35} $&$  3.0 $&$ ^{+1.2}_{-1.3} $&$    100.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.73 $ \\
$ 900835$&$  266.49982 $&$   -28.887201 $&$  3930 $&$ ^{+340}_{-340} $&$  0.62 $&$ ^{+0.41}_{-0.41} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -10.2 $&$ ^{+13.8}_{-13.8} $&$  13.10 $ \\
$ 900836$&$  266.49762 $&$   -28.879457 $&$  4150 $&$ ^{+290}_{-280} $&$  0.50 $&$ ^{+0.35}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.0} $&$     25.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.91 $ \\
$ 900841$&$  266.50031 $&$   -28.880493 $&$  4060 $&$ ^{+280}_{-280} $&$  0.48 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -26.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.74 $ \\
$ 900843$&$  266.50195 $&$   -28.877428 $&$  3710 $&$ ^{+280}_{-280} $&$  0.82 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     58.0 $&$ ^{+ 3.1}_{- 3.1} $&$  13.61 $ \\
$ 900846$&$  266.49857 $&$   -28.888067 $&$  4290 $&$ ^{+310}_{-300} $&$  0.14 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     15.4 $&$ ^{+ 3.1}_{- 3.1} $&$  13.04 $ \\
$ 900849$&$  266.50375 $&$   -28.880493 $&$  3880 $&$ ^{+280}_{-280} $&$  0.92 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -68.4 $&$ ^{+ 3.1}_{- 3.1} $&$  13.08 $ \\
$ 900862$&$  266.50125 $&$   -28.876791 $&$  4400 $&$ ^{+310}_{-310} $&$ -0.20 $&$ ^{+0.37}_{-0.36} $&$  4.3 $&$ ^{+1.1}_{-1.0} $&$     51.5 $&$ ^{+ 5.5}_{- 4.8} $&$  13.27 $ \\
$ 900878$&$  266.49841 $&$   -28.877047 $&$  4140 $&$ ^{+300}_{-310} $&$  0.03 $&$ ^{+0.36}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.2} $&$    -55.9 $&$ ^{+ 5.7}_{- 6.2} $&$  13.03 $ \\
$ 900883$&$  266.49881 $&$   -28.885130 $&$  3700 $&$ ^{+300}_{-300} $&$  0.81 $&$ ^{+0.36}_{-0.34} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     21.0 $&$ ^{+ 5.2}_{- 5.1} $&$  13.21 $ \\
$ 900910$&$  266.49362 $&$   -28.886799 $&$  4750 $&$ ^{+320}_{-330} $&$  0.38 $&$ ^{+0.36}_{-0.37} $&$  2.6 $&$ ^{+1.1}_{-1.2} $&$    127.4 $&$ ^{+ 3.3}_{- 3.6} $&$  13.29 $ \\
$ 900926$&$  266.49734 $&$   -28.879450 $&$  3870 $&$ ^{+280}_{-280} $&$  0.92 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -30.3 $&$ ^{+ 3.1}_{- 3.1} $&$  12.84 $ \\
$ 900941$&$  266.49857 $&$   -28.874098 $&$  4080 $&$ ^{+280}_{-280} $&$ -0.05 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     53.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.85 $ \\
$ 900954$&$  266.49530 $&$   -28.882912 $&$  3870 $&$ ^{+280}_{-280} $&$  0.64 $&$ ^{+0.36}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     63.0 $&$ ^{+ 4.8}_{- 4.6} $&$  12.96 $ \\
$ 900957$&$  266.49146 $&$   -28.886953 $&$  4330 $&$ ^{+300}_{-290} $&$  0.02 $&$ ^{+0.36}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.2} $&$     12.7 $&$ ^{+ 4.5}_{- 4.5} $&$  13.02 $ \\
$ 900987$&$  266.50861 $&$   -28.874788 $&$  3700 $&$ ^{+280}_{-280} $&$  0.13 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     78.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.61 $ \\
$ 900996$&$  266.50293 $&$   -28.877228 $&$  4250 $&$ ^{+300}_{-300} $&$ -0.37 $&$ ^{+0.35}_{-0.35} $&$  4.2 $&$ ^{+1.1}_{-1.0} $&$     11.4 $&$ ^{+ 4.1}_{- 4.1} $&$  13.25 $ \\
$ 901010$&$  266.49994 $&$   -28.887358 $&$  3780 $&$ ^{+300}_{-290} $&$  0.88 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     -8.6 $&$ ^{+ 3.1}_{- 3.1} $&$  13.03 $ \\
$ 901151$&$  266.50772 $&$   -28.879545 $&$  4120 $&$ ^{+290}_{-310} $&$  0.75 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     55.9 $&$ ^{+ 3.1}_{- 3.1} $&$  13.61 $ \\
$ 901154$&$  266.50327 $&$   -28.884708 $&$  4260 $&$ ^{+300}_{-300} $&$  0.40 $&$ ^{+0.36}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.1} $&$      4.7 $&$ ^{+ 3.1}_{- 3.1} $&$  13.01 $ \\
$ 901175$&$  266.50500 $&$   -28.877094 $&$  3890 $&$ ^{+280}_{-280} $&$  0.51 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     19.4 $&$ ^{+ 3.1}_{- 3.1} $&$  13.27 $ \\
$ 901193$&$  266.49963 $&$   -28.878111 $&$  3840 $&$ ^{+290}_{-280} $&$  0.87 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     92.2 $&$ ^{+ 3.1}_{- 3.1} $&$  13.12 $ \\
$ 901202$&$  266.50113 $&$   -28.876453 $&$  4030 $&$ ^{+300}_{-300} $&$  0.45 $&$ ^{+0.37}_{-0.37} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     45.8 $&$ ^{+ 3.1}_{- 3.1} $&$  13.16 $ \\
$ 901241$&$  266.50153 $&$   -28.878544 $&$  3780 $&$ ^{+370}_{-370} $&$ -0.42 $&$ ^{+0.56}_{-0.56} $&$  1.4 $&$ ^{+1.6}_{-1.6} $&$   -143.5 $&$ ^{+ 4.6}_{- 4.6} $&$  10.84 $ \\
$ 901250$&$  266.49741 $&$   -28.883760 $&$  3950 $&$ ^{+280}_{-280} $&$  0.80 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     72.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.52 $ \\
$ 901262$&$  266.50284 $&$   -28.882147 $&$  3850 $&$ ^{+340}_{-270} $&$  0.28 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -21.9 $&$ ^{+ 3.1}_{- 3.1} $&$  10.81 $ \\
$ 901268$&$  266.50290 $&$   -28.878580 $&$  4380 $&$ ^{+290}_{-290} $&$ -0.16 $&$ ^{+0.34}_{-0.34} $&$  4.3 $&$ ^{+1.0}_{-1.0} $&$     22.7 $&$ ^{+ 1.9}_{- 1.9} $&$  12.66 $ \\
$ 901369$&$  266.49548 $&$   -28.885967 $&$  3420 $&$ ^{+280}_{-280} $&$  0.91 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     37.8 $&$ ^{+ 3.1}_{- 3.1} $&$  13.62 $ \\
$ 901370$&$  266.50836 $&$   -28.874901 $&$  4130 $&$ ^{+290}_{-290} $&$ -0.19 $&$ ^{+0.36}_{-0.35} $&$  2.6 $&$ ^{+1.1}_{-1.1} $&$    165.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.02 $ \\
$ 901387$&$  266.50488 $&$   -28.872826 $&$  3870 $&$ ^{+280}_{-280} $&$  0.35 $&$ ^{+0.36}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     61.3 $&$ ^{+ 3.1}_{- 3.1} $&$  14.20 $ \\
$ 901524$&$  266.49603 $&$   -28.880342 $&$  3850 $&$ ^{+280}_{-280} $&$  0.68 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     17.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.18 $ \\
$ 901572$&$  266.50092 $&$   -28.880407 $&$  3970 $&$ ^{+280}_{-280} $&$  0.40 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.1} $&$     60.3 $&$ ^{+ 3.1}_{- 3.1} $&$  12.96 $ \\
$ 901763$&$  266.50900 $&$   -28.882393 $&$  3850 $&$ ^{+280}_{-280} $&$  0.47 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$      6.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.66 $ \\
$ 901767$&$  266.51166 $&$   -28.878635 $&$  3550 $&$ ^{+280}_{-280} $&$  0.70 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -90.6 $&$ ^{+ 3.1}_{- 3.1} $&$  11.34 $ \\
$ 901799$&$  266.50491 $&$   -28.888147 $&$  3870 $&$ ^{+280}_{-280} $&$  0.22 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     46.5 $&$ ^{+ 3.1}_{- 3.1} $&$  11.60 $ \\
$ 901803$&$  266.50906 $&$   -28.881784 $&$  3940 $&$ ^{+280}_{-280} $&$  0.61 $&$ ^{+0.35}_{-0.34} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     72.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.34 $ \\
$ 901813$&$  266.50787 $&$   -28.883383 $&$  3940 $&$ ^{+280}_{-280} $&$  0.86 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -55.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.04 $ \\
$ 901822$&$  266.50797 $&$   -28.883654 $&$  4300 $&$ ^{+310}_{-290} $&$  0.06 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$   -141.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.52 $ \\
$ 901866$&$  266.50641 $&$   -28.885857 $&$  3890 $&$ ^{+280}_{-280} $&$ -0.04 $&$ ^{+0.34}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     76.8 $&$ ^{+ 3.1}_{- 3.1} $&$  11.92 $ \\
$ 901953$&$  266.50986 $&$   -28.881079 $&$  4280 $&$ ^{+300}_{-300} $&$  0.22 $&$ ^{+0.35}_{-0.36} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$    180.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.86 $ \\
$ 902411$&$  266.50494 $&$   -28.876884 $&$  3860 $&$ ^{+280}_{-280} $&$  0.57 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$      1.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.51 $ \\
$ 902412$&$  266.49615 $&$   -28.886969 $&$  3860 $&$ ^{+280}_{-280} $&$  0.71 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     31.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.92 $ \\
$ 902414$&$  266.50150 $&$   -28.879263 $&$  4350 $&$ ^{+290}_{-290} $&$  0.41 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$      0.8 $&$ ^{+ 6.0}_{- 7.1} $&$  12.33 $ \\
$ 902416$&$  266.50159 $&$   -28.881025 $&$  3980 $&$ ^{+280}_{-280} $&$  0.39 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -67.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.75 $ \\
$ 902420$&$  266.50375 $&$   -28.884890 $&$  4330 $&$ ^{+300}_{-290} $&$  0.38 $&$ ^{+0.35}_{-0.36} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     15.1 $&$ ^{+ 3.1}_{- 3.1} $&$  13.16 $ \\
$ 902425$&$  266.50269 $&$   -28.878908 $&$  3900 $&$ ^{+280}_{-280} $&$  0.72 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    222.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.47 $ \\
$ 902428$&$  266.50143 $&$   -28.877951 $&$  4140 $&$ ^{+290}_{-300} $&$  0.23 $&$ ^{+0.35}_{-0.35} $&$  3.7 $&$ ^{+1.4}_{-1.1} $&$   -197.3 $&$ ^{+ 3.1}_{- 3.1} $&$  12.85 $ \\
$ 902431$&$  266.50266 $&$   -28.880396 $&$  3800 $&$ ^{+280}_{-280} $&$  0.94 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -43.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.44 $ \\
$ 902434$&$  266.50113 $&$   -28.871828 $&$  4040 $&$ ^{+280}_{-290} $&$  0.07 $&$ ^{+0.37}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.1} $&$     77.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.78 $ \\
$ 902620$&$  266.50522 $&$   -28.879269 $&$  3870 $&$ ^{+290}_{-300} $&$  0.72 $&$ ^{+0.36}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.1} $&$    -18.0 $&$ ^{+ 3.3}_{- 3.3} $&$  13.49 $ \\
$ 902646$&$  266.49808 $&$   -28.882999 $&$  4230 $&$ ^{+280}_{-280} $&$ -0.03 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$   -112.7 $&$ ^{+ 3.1}_{- 3.1} $&$  13.89 $ \\
$ 902903$&$  266.50864 $&$   -28.882729 $&$  3610 $&$ ^{+280}_{-280} $&$  0.25 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$      2.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.86 $ \\
$ 903001$&$  266.50357 $&$   -28.888054 $&$  4220 $&$ ^{+310}_{-310} $&$  0.13 $&$ ^{+0.38}_{-0.37} $&$  2.8 $&$ ^{+1.1}_{-1.1} $&$     24.4 $&$ ^{+ 4.9}_{- 5.1} $&$  13.53 $ \\
$ 910000$&$  266.50089 $&$   -28.870626 $&$  3540 $&$ ^{+280}_{-280} $&$ -0.18 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    149.2 $&$ ^{+ 3.1}_{- 3.1} $&$   8.88 $ \\
$1000167$&$  266.33325 $&$   -29.130653 $&$  3410 $&$ ^{+270}_{-270} $&$  0.24 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     11.3 $&$ ^{+ 1.1}_{- 1.1} $&$   8.32 $ \\
$1000169$&$  266.32849 $&$   -29.139717 $&$  3890 $&$ ^{+270}_{-270} $&$  0.09 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -34.9 $&$ ^{+ 6.4}_{- 6.4} $&$  10.07 $ \\
$1000170$&$  266.33423 $&$   -29.132572 $&$  3970 $&$ ^{+280}_{-280} $&$ -0.35 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -37.0 $&$ ^{+ 3.1}_{- 3.1} $&$  10.34 $ \\
$1000171$&$  266.32870 $&$   -29.139894 $&$  3610 $&$ ^{+280}_{-280} $&$  0.42 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    125.9 $&$ ^{+ 3.1}_{- 3.1} $&$  10.29 $ \\
$1000173$&$  266.33246 $&$   -29.132133 $&$  3900 $&$ ^{+280}_{-280} $&$ -0.28 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$   -254.0 $&$ ^{+ 3.1}_{- 3.1} $&$  10.69 $ \\
$1000177$&$  266.33197 $&$   -29.135801 $&$  3380 $&$ ^{+290}_{-290} $&$  0.33 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -85.7 $&$ ^{+ 0.5}_{- 0.5} $&$   9.39 $ \\
$1000181$&$  266.33438 $&$   -29.130856 $&$  4040 $&$ ^{+300}_{-300} $&$ -0.20 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -91.4 $&$ ^{+ 2.4}_{- 2.4} $&$  10.24 $ \\
$1000187$&$  266.32806 $&$   -29.138783 $&$  3910 $&$ ^{+280}_{-270} $&$  0.10 $&$ ^{+0.33}_{-0.34} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$     23.8 $&$ ^{+ 1.5}_{- 1.5} $&$  11.70 $ \\
$1000188$&$  266.33276 $&$   -29.133636 $&$  3460 $&$ ^{+280}_{-280} $&$  0.24 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -36.9 $&$ ^{+ 3.1}_{- 3.1} $&$  10.67 $ \\
$1000205$&$  266.32852 $&$   -29.135332 $&$  3630 $&$ ^{+280}_{-280} $&$ -0.12 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -111.9 $&$ ^{+ 3.1}_{- 3.1} $&$   8.09 $ \\
$1000213$&$  266.33005 $&$   -29.124704 $&$  3540 $&$ ^{+290}_{-290} $&$  0.19 $&$ ^{+0.38}_{-0.38} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    137.5 $&$ ^{+ 2.1}_{- 2.1} $&$   9.12 $ \\
$1000217$&$  266.32465 $&$   -29.133801 $&$  3960 $&$ ^{+280}_{-280} $&$ -1.13 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$   -138.8 $&$ ^{+ 3.1}_{- 3.1} $&$   9.78 $ \\
$1000220$&$  266.32715 $&$   -29.130384 $&$  3520 $&$ ^{+300}_{-300} $&$ -0.08 $&$ ^{+0.49}_{-0.49} $&$  0.3 $&$ ^{+1.1}_{-1.1} $&$    -28.4 $&$ ^{+ 4.9}_{- 4.9} $&$   8.20 $ \\
$1000224$&$  266.33511 $&$   -29.125818 $&$  3650 $&$ ^{+290}_{-290} $&$ -0.14 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     24.8 $&$ ^{+ 3.2}_{- 3.2} $&$   9.38 $ \\
$1000226$&$  266.32181 $&$   -29.135309 $&$  3440 $&$ ^{+280}_{-280} $&$  0.30 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$      0.5 $&$ ^{+ 3.1}_{- 3.1} $&$   8.33 $ \\
$1000237$&$  266.32339 $&$   -29.131287 $&$  3600 $&$ ^{+280}_{-280} $&$  0.32 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     44.0 $&$ ^{+ 3.1}_{- 3.1} $&$   9.95 $ \\
$1000238$&$  266.33133 $&$   -29.125881 $&$  3920 $&$ ^{+280}_{-280} $&$ -1.01 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -15.8 $&$ ^{+ 1.7}_{- 1.7} $&$   9.48 $ \\
$1000240$&$  266.32083 $&$   -29.133018 $&$  3840 $&$ ^{+290}_{-290} $&$ -0.32 $&$ ^{+0.36}_{-0.36} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$    111.5 $&$ ^{+ 8.0}_{- 8.0} $&$   9.68 $ \\
$1000244$&$  266.32556 $&$   -29.133463 $&$  3590 $&$ ^{+270}_{-270} $&$ -0.20 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -85.7 $&$ ^{+ 4.8}_{- 4.8} $&$   9.29 $ \\
$1000248$&$  266.32327 $&$   -29.134521 $&$  3800 $&$ ^{+300}_{-300} $&$  0.11 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -41.4 $&$ ^{+ 0.4}_{- 0.5} $&$  10.09 $ \\
$1000251$&$  266.33282 $&$   -29.124626 $&$  3430 $&$ ^{+280}_{-280} $&$  0.36 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$   -100.5 $&$ ^{+ 3.1}_{- 3.1} $&$   9.18 $ \\
$1000256$&$  266.32581 $&$   -29.125874 $&$  4270 $&$ ^{+280}_{-280} $&$ -0.31 $&$ ^{+0.35}_{-0.35} $&$  3.7 $&$ ^{+1.0}_{-1.0} $&$   -189.2 $&$ ^{+ 3.1}_{- 3.1} $&$  10.66 $ \\
$1000257$&$  266.32748 $&$   -29.128748 $&$  3610 $&$ ^{+360}_{-360} $&$  0.19 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$   -119.0 $&$ ^{+ 3.2}_{- 3.2} $&$   9.24 $ \\
$1000258$&$  266.32172 $&$   -29.133629 $&$  2780 $&$ ^{+390}_{-390} $&$ -0.62 $&$ ^{+0.73}_{-0.73} $&$  2.1 $&$ ^{+2.8}_{-2.8} $&$     -0.5 $&$ ^{+ 3.1}_{- 3.1} $&$   8.16 $ \\
$1000260$&$  266.32697 $&$   -29.128038 $&$  3500 $&$ ^{+300}_{-300} $&$  0.22 $&$ ^{+0.49}_{-0.49} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -86.4 $&$ ^{+ 5.7}_{- 5.7} $&$   9.32 $ \\
$1000263$&$  266.33325 $&$   -29.126732 $&$  3660 $&$ ^{+410}_{-410} $&$  0.19 $&$ ^{+0.36}_{-0.36} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -140.6 $&$ ^{+ 0.4}_{- 0.4} $&$  10.79 $ \\
$1000264$&$  266.32016 $&$   -29.132912 $&$  3440 $&$ ^{+280}_{-280} $&$  0.19 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -64.2 $&$ ^{+ 1.0}_{- 1.0} $&$   9.25 $ \\
$1000268$&$  266.32407 $&$   -29.127092 $&$  3440 $&$ ^{+280}_{-280} $&$  0.24 $&$ ^{+0.36}_{-0.36} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -69.5 $&$ ^{+ 7.8}_{- 7.8} $&$   9.11 $ \\
$1000269$&$  266.32458 $&$   -29.137293 $&$  3890 $&$ ^{+270}_{-270} $&$  0.05 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     -6.3 $&$ ^{+ 2.6}_{- 2.6} $&$  10.05 $ \\
$1000271$&$  266.31937 $&$   -29.131971 $&$  3400 $&$ ^{+270}_{-270} $&$  0.50 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     16.6 $&$ ^{+ 3.0}_{- 3.0} $&$   8.97 $ \\
$1000273$&$  266.32318 $&$   -29.130936 $&$  3370 $&$ ^{+280}_{-280} $&$  0.47 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$      7.3 $&$ ^{+ 9.3}_{- 9.3} $&$   9.72 $ \\
$1000275$&$  266.32483 $&$   -29.128569 $&$  3620 $&$ ^{+350}_{-350} $&$  0.41 $&$ ^{+0.51}_{-0.51} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -23.8 $&$ ^{+ 1.9}_{- 1.9} $&$  10.86 $ \\
$1000280$&$  266.32068 $&$   -29.134422 $&$  3780 $&$ ^{+300}_{-300} $&$  0.20 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -22.3 $&$ ^{+ 1.4}_{- 1.4} $&$  10.12 $ \\
$1000283$&$  266.32950 $&$   -29.128658 $&$  3520 $&$ ^{+290}_{-290} $&$  0.25 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -72.4 $&$ ^{+ 1.6}_{- 1.6} $&$   9.82 $ \\
$1000292$&$  266.32272 $&$   -29.132542 $&$  3930 $&$ ^{+280}_{-280} $&$ -0.16 $&$ ^{+0.35}_{-0.35} $&$  2.6 $&$ ^{+1.0}_{-1.0} $&$    115.0 $&$ ^{+ 3.1}_{- 3.1} $&$  10.08 $ \\
$1000302$&$  266.31918 $&$   -29.135298 $&$  4310 $&$ ^{+290}_{-290} $&$ -0.24 $&$ ^{+0.40}_{-0.40} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     67.5 $&$ ^{+ 1.0}_{- 1.0} $&$  10.76 $ \\
$1000313$&$  266.32779 $&$   -29.138603 $&$  3850 $&$ ^{+270}_{-270} $&$  0.14 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -87.5 $&$ ^{+ 4.1}_{- 4.1} $&$  11.02 $ \\
$1000315$&$  266.32474 $&$   -29.135750 $&$  3870 $&$ ^{+270}_{-270} $&$  0.20 $&$ ^{+0.33}_{-0.33} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$    -32.7 $&$ ^{+ 1.1}_{- 1.1} $&$  10.40 $ \\
$1000316$&$  266.32950 $&$   -29.132811 $&$  3740 $&$ ^{+300}_{-290} $&$  0.41 $&$ ^{+0.38}_{-0.37} $&$  0.9 $&$ ^{+1.1}_{-1.1} $&$     75.2 $&$ ^{+ 3.1}_{- 3.1} $&$  11.50 $ \\
$1000317$&$  266.32172 $&$   -29.137766 $&$  3540 $&$ ^{+340}_{-340} $&$  0.43 $&$ ^{+0.34}_{-0.34} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -47.1 $&$ ^{+ 6.2}_{- 6.2} $&$  10.00 $ \\
$1000318$&$  266.32858 $&$   -29.138018 $&$  3900 $&$ ^{+270}_{-270} $&$ -0.16 $&$ ^{+0.34}_{-0.34} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -20.5 $&$ ^{+ 2.4}_{- 2.4} $&$  11.92 $ \\
$1000320$&$  266.32846 $&$   -29.132357 $&$  3410 $&$ ^{+280}_{-280} $&$  0.66 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -187.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.11 $ \\
$1000322$&$  266.32870 $&$   -29.138678 $&$  3460 $&$ ^{+290}_{-290} $&$  0.38 $&$ ^{+0.36}_{-0.36} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     78.9 $&$ ^{+ 4.9}_{- 4.9} $&$   9.70 $ \\
$1000332$&$  266.32086 $&$   -29.130407 $&$  3890 $&$ ^{+280}_{-280} $&$ -0.07 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -66.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.32 $ \\
$1000340$&$  266.33267 $&$   -29.129375 $&$  4010 $&$ ^{+300}_{-310} $&$ -1.15 $&$ ^{+0.37}_{-0.41} $&$  1.1 $&$ ^{+1.2}_{-1.2} $&$    -99.9 $&$ ^{+ 8.4}_{- 8.5} $&$  11.95 $ \\
$1000343$&$  266.33057 $&$   -29.125172 $&$  3800 $&$ ^{+320}_{-320} $&$  0.12 $&$ ^{+0.41}_{-0.41} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -92.0 $&$ ^{+ 3.2}_{- 3.2} $&$  11.17 $ \\
$1000352$&$  266.33365 $&$   -29.127872 $&$  4070 $&$ ^{+280}_{-280} $&$ -0.28 $&$ ^{+0.32}_{-0.32} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     -7.3 $&$ ^{+ 1.3}_{- 1.3} $&$  11.65 $ \\
$1000355$&$  266.33066 $&$   -29.125463 $&$  5030 $&$ ^{+280}_{-280} $&$ -0.51 $&$ ^{+0.35}_{-0.35} $&$  2.5 $&$ ^{+1.0}_{-1.0} $&$   -102.7 $&$ ^{+ 3.4}_{- 3.5} $&$  11.79 $ \\
$1000356$&$  266.33212 $&$   -29.135258 $&$  3490 $&$ ^{+280}_{-280} $&$  0.25 $&$ ^{+0.40}_{-0.40} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -40.2 $&$ ^{+ 5.5}_{- 5.5} $&$  10.83 $ \\
$1000359$&$  266.33197 $&$   -29.130289 $&$  3650 $&$ ^{+410}_{-410} $&$  0.29 $&$ ^{+0.34}_{-0.34} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -81.3 $&$ ^{+ 0.5}_{- 0.4} $&$  10.46 $ \\
$1000361$&$  266.32480 $&$   -29.134541 $&$  4050 $&$ ^{+310}_{-310} $&$ -0.16 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -19.1 $&$ ^{+ 6.9}_{- 6.9} $&$  10.72 $ \\
$1000364$&$  266.32932 $&$   -29.133224 $&$  4630 $&$ ^{+280}_{-280} $&$  0.39 $&$ ^{+0.35}_{-0.35} $&$  3.7 $&$ ^{+1.0}_{-1.0} $&$    -63.5 $&$ ^{+ 3.1}_{- 3.1} $&$  11.86 $ \\
$1000371$&$  266.33023 $&$   -29.130207 $&$  3610 $&$ ^{+280}_{-280} $&$ -0.94 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    150.8 $&$ ^{+ 3.1}_{- 3.1} $&$   9.37 $ \\
$1000372$&$  266.31671 $&$   -29.137093 $&$  3730 $&$ ^{+340}_{-340} $&$  0.39 $&$ ^{+0.38}_{-0.38} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -56.2 $&$ ^{+ 3.1}_{- 3.1} $&$  11.04 $ \\
$1000375$&$  266.32642 $&$   -29.132233 $&$  3600 $&$ ^{+370}_{-370} $&$  0.01 $&$ ^{+0.68}_{-0.68} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    263.3 $&$ ^{+ 1.1}_{- 1.1} $&$   9.55 $ \\
$1000380$&$  266.33066 $&$   -29.124325 $&$  3990 $&$ ^{+280}_{-280} $&$ -0.14 $&$ ^{+0.36}_{-0.36} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -79.7 $&$ ^{+ 3.7}_{- 3.7} $&$  11.83 $ \\
$1000389$&$  266.32611 $&$   -29.122555 $&$  4310 $&$ ^{+280}_{-280} $&$ -0.59 $&$ ^{+0.35}_{-0.35} $&$  4.0 $&$ ^{+1.0}_{-1.0} $&$    -29.4 $&$ ^{+ 3.1}_{- 3.1} $&$  11.03 $ \\
$1000392$&$  266.32538 $&$   -29.134829 $&$  3760 $&$ ^{+310}_{-310} $&$  0.11 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     -0.7 $&$ ^{+ 1.5}_{- 1.5} $&$  10.51 $ \\
$1000394$&$  266.32883 $&$   -29.123379 $&$  3870 $&$ ^{+280}_{-270} $&$  0.00 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$      3.0 $&$ ^{+ 1.9}_{- 1.9} $&$  11.29 $ \\
$1000398$&$  266.33072 $&$   -29.127529 $&$  3750 $&$ ^{+340}_{-340} $&$  0.04 $&$ ^{+0.36}_{-0.36} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     -9.3 $&$ ^{+ 2.1}_{- 2.1} $&$  11.00 $ \\
$1000400$&$  266.33334 $&$   -29.129461 $&$  3950 $&$ ^{+270}_{-270} $&$ -0.17 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -79.2 $&$ ^{+ 1.5}_{- 1.5} $&$  11.09 $ \\
$1000422$&$  266.32913 $&$   -29.129253 $&$  3790 $&$ ^{+290}_{-290} $&$  0.15 $&$ ^{+0.40}_{-0.40} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -14.9 $&$ ^{+ 6.6}_{- 6.6} $&$  11.22 $ \\
$1000423$&$  266.32376 $&$   -29.132254 $&$  4130 $&$ ^{+290}_{-300} $&$  0.50 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -50.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.16 $ \\
$1000424$&$  266.32654 $&$   -29.131292 $&$  3480 $&$ ^{+280}_{-280} $&$  0.31 $&$ ^{+0.37}_{-0.37} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -184.2 $&$ ^{+ 2.4}_{- 2.4} $&$  11.16 $ \\
$1000426$&$  266.32272 $&$   -29.139215 $&$  4060 $&$ ^{+300}_{-300} $&$ -0.50 $&$ ^{+0.35}_{-0.35} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$    -85.3 $&$ ^{+ 4.7}_{- 4.7} $&$  10.26 $ \\
$1000429$&$  266.32535 $&$   -29.130953 $&$  3780 $&$ ^{+290}_{-290} $&$  0.14 $&$ ^{+0.34}_{-0.34} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -30.4 $&$ ^{+ 4.3}_{- 4.3} $&$  11.42 $ \\
$1000433$&$  266.32272 $&$   -29.127054 $&$  4040 $&$ ^{+280}_{-290} $&$  0.32 $&$ ^{+0.35}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.1} $&$    -53.6 $&$ ^{+ 3.1}_{- 3.1} $&$  12.27 $ \\
$1000436$&$  266.32639 $&$   -29.130247 $&$  3510 $&$ ^{+270}_{-270} $&$  0.02 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    166.1 $&$ ^{+ 1.9}_{- 1.9} $&$   9.63 $ \\
$1000437$&$  266.32401 $&$   -29.131807 $&$  3970 $&$ ^{+280}_{-280} $&$  0.41 $&$ ^{+0.37}_{-0.33} $&$  1.3 $&$ ^{+1.0}_{-1.1} $&$    -16.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.30 $ \\
$1000438$&$  266.32684 $&$   -29.121927 $&$  3670 $&$ ^{+280}_{-280} $&$  0.12 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     26.3 $&$ ^{+ 6.2}_{- 6.2} $&$  10.62 $ \\
$1000440$&$  266.33026 $&$   -29.124203 $&$  3890 $&$ ^{+280}_{-280} $&$  0.13 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    188.2 $&$ ^{+ 3.1}_{- 3.1} $&$  11.46 $ \\
$1000443$&$  266.32611 $&$   -29.123983 $&$  3460 $&$ ^{+280}_{-280} $&$  0.26 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -82.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.34 $ \\
$1000444$&$  266.32758 $&$   -29.124228 $&$  4030 $&$ ^{+280}_{-280} $&$ -0.18 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -76.8 $&$ ^{+ 3.1}_{- 3.1} $&$  11.79 $ \\
$1000447$&$  266.31818 $&$   -29.136040 $&$  4210 $&$ ^{+320}_{-300} $&$  0.59 $&$ ^{+0.36}_{-0.35} $&$  3.8 $&$ ^{+1.3}_{-1.1} $&$   -103.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.17 $ \\
$1000454$&$  266.33310 $&$   -29.125591 $&$  3630 $&$ ^{+270}_{-270} $&$  0.31 $&$ ^{+0.36}_{-0.36} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     53.4 $&$ ^{+ 0.7}_{- 0.7} $&$  10.47 $ \\
$1000456$&$  266.32269 $&$   -29.137798 $&$  3410 $&$ ^{+270}_{-270} $&$  0.44 $&$ ^{+0.32}_{-0.32} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     54.2 $&$ ^{+ 3.4}_{- 3.4} $&$   9.72 $ \\
$1000468$&$  266.32831 $&$   -29.127831 $&$  3850 $&$ ^{+280}_{-270} $&$  0.11 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -261.1 $&$ ^{+ 2.5}_{- 2.5} $&$  11.08 $ \\
$1000474$&$  266.33246 $&$   -29.129946 $&$  4080 $&$ ^{+280}_{-300} $&$  0.45 $&$ ^{+0.35}_{-0.35} $&$  3.6 $&$ ^{+1.2}_{-1.1} $&$    -83.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.42 $ \\
$1000476$&$  266.32974 $&$   -29.132177 $&$  3850 $&$ ^{+280}_{-280} $&$  0.29 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$      8.5 $&$ ^{+ 3.1}_{- 3.1} $&$  10.81 $ \\
$1000479$&$  266.32047 $&$   -29.132179 $&$  3800 $&$ ^{+280}_{-280} $&$ -0.22 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -137.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.23 $ \\
$1000480$&$  266.32205 $&$   -29.138348 $&$  3810 $&$ ^{+270}_{-270} $&$  0.22 $&$ ^{+0.53}_{-0.53} $&$  0.5 $&$ ^{+1.1}_{-1.1} $&$    -54.3 $&$ ^{+ 2.4}_{- 2.4} $&$  11.61 $ \\
$1000483$&$  266.32288 $&$   -29.127502 $&$  3920 $&$ ^{+270}_{-270} $&$ -0.15 $&$ ^{+0.34}_{-0.34} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -10.0 $&$ ^{+ 1.0}_{- 1.1} $&$  11.85 $ \\
$1000486$&$  266.32455 $&$   -29.135973 $&$  3790 $&$ ^{+310}_{-310} $&$  0.12 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -20.8 $&$ ^{+ 2.6}_{- 2.6} $&$  10.56 $ \\
$1000487$&$  266.31830 $&$   -29.136662 $&$  3890 $&$ ^{+280}_{-280} $&$ -0.52 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -107.5 $&$ ^{+ 3.1}_{- 3.1} $&$  10.91 $ \\
$1000489$&$  266.32785 $&$   -29.123110 $&$  3830 $&$ ^{+280}_{-280} $&$ -0.14 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -89.6 $&$ ^{+ 3.1}_{- 3.1} $&$  11.74 $ \\
$1000497$&$  266.32767 $&$   -29.122442 $&$  3910 $&$ ^{+280}_{-280} $&$ -0.48 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -146.4 $&$ ^{+ 3.1}_{- 3.1} $&$  10.97 $ \\
$1000500$&$  266.32950 $&$   -29.124216 $&$  3440 $&$ ^{+270}_{-270} $&$  0.31 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     61.3 $&$ ^{+ 1.7}_{- 1.7} $&$  10.58 $ \\
$1000501$&$  266.32150 $&$   -29.131865 $&$  3990 $&$ ^{+310}_{-280} $&$  0.18 $&$ ^{+0.34}_{-0.37} $&$  0.4 $&$ ^{+1.0}_{-1.1} $&$    -13.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.79 $ \\
$1000505$&$  266.33347 $&$   -29.125202 $&$  3870 $&$ ^{+280}_{-280} $&$  0.08 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     88.5 $&$ ^{+ 3.1}_{- 3.1} $&$  11.52 $ \\
$1000508$&$  266.32401 $&$   -29.139496 $&$  4310 $&$ ^{+390}_{-390} $&$  0.20 $&$ ^{+0.34}_{-0.34} $&$  2.4 $&$ ^{+1.0}_{-1.0} $&$    -64.3 $&$ ^{+ 4.4}_{- 4.4} $&$  12.06 $ \\
$1000510$&$  266.32132 $&$   -29.131372 $&$  3540 $&$ ^{+280}_{-280} $&$  0.95 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -52.2 $&$ ^{+ 3.1}_{- 3.1} $&$  11.63 $ \\
$1000513$&$  266.32349 $&$   -29.127752 $&$  4310 $&$ ^{+320}_{-320} $&$ -0.04 $&$ ^{+0.38}_{-0.38} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -99.1 $&$ ^{+ 1.7}_{- 1.8} $&$  11.78 $ \\
$1000517$&$  266.32227 $&$   -29.139709 $&$  3890 $&$ ^{+270}_{-270} $&$  0.03 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     -3.9 $&$ ^{+ 1.1}_{- 1.1} $&$  11.26 $ \\
$1000519$&$  266.32690 $&$   -29.126619 $&$  4220 $&$ ^{+310}_{-310} $&$  0.31 $&$ ^{+0.38}_{-0.38} $&$  2.4 $&$ ^{+1.0}_{-1.0} $&$    -77.7 $&$ ^{+ 7.2}_{- 7.2} $&$  12.08 $ \\
$1000522$&$  266.32913 $&$   -29.124439 $&$  3920 $&$ ^{+300}_{-290} $&$  0.86 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -64.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.71 $ \\
$1000523$&$  266.32703 $&$   -29.125278 $&$  3470 $&$ ^{+280}_{-280} $&$  0.63 $&$ ^{+0.47}_{-0.47} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -64.1 $&$ ^{+ 1.9}_{- 1.9} $&$  11.63 $ \\
$1000528$&$  266.32974 $&$   -29.124201 $&$  3650 $&$ ^{+270}_{-270} $&$  0.48 $&$ ^{+0.34}_{-0.34} $&$  0.6 $&$ ^{+1.2}_{-1.2} $&$    -14.4 $&$ ^{+ 2.5}_{- 2.5} $&$  11.03 $ \\
$1000535$&$  266.32822 $&$   -29.131153 $&$  3910 $&$ ^{+280}_{-280} $&$  0.19 $&$ ^{+0.34}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -14.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.93 $ \\
$1000538$&$  266.32581 $&$   -29.132259 $&$  4000 $&$ ^{+280}_{-290} $&$  0.36 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     -2.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.45 $ \\
$1000540$&$  266.32373 $&$   -29.133348 $&$  4340 $&$ ^{+320}_{-300} $&$  0.06 $&$ ^{+0.36}_{-0.36} $&$  0.4 $&$ ^{+1.0}_{-1.1} $&$    -86.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.51 $ \\
$1000542$&$  266.32275 $&$   -29.130119 $&$  3910 $&$ ^{+280}_{-280} $&$  0.05 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -34.5 $&$ ^{+ 3.1}_{- 3.1} $&$  11.67 $ \\
$1000546$&$  266.32068 $&$   -29.135736 $&$  4030 $&$ ^{+280}_{-280} $&$ -0.05 $&$ ^{+0.35}_{-0.35} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$    -51.9 $&$ ^{+ 3.1}_{- 3.1} $&$  11.66 $ \\
$1000553$&$  266.32040 $&$   -29.132763 $&$  3700 $&$ ^{+280}_{-280} $&$ -0.15 $&$ ^{+0.38}_{-0.38} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -84.4 $&$ ^{+12.5}_{-12.5} $&$  11.80 $ \\
$1000568$&$  266.32242 $&$   -29.128492 $&$  3880 $&$ ^{+270}_{-270} $&$ -0.03 $&$ ^{+0.39}_{-0.39} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -28.1 $&$ ^{+ 0.9}_{- 0.9} $&$  11.72 $ \\
$1000571$&$  266.32639 $&$   -29.126987 $&$  4540 $&$ ^{+290}_{-290} $&$  0.18 $&$ ^{+0.35}_{-0.35} $&$  4.4 $&$ ^{+1.0}_{-1.0} $&$     31.8 $&$ ^{+ 4.6}_{- 4.4} $&$  12.86 $ \\
$1000573$&$  266.32639 $&$   -29.129797 $&$  3880 $&$ ^{+280}_{-280} $&$ -0.04 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     -0.9 $&$ ^{+ 3.1}_{- 3.1} $&$  11.91 $ \\
$1000574$&$  266.33307 $&$   -29.127287 $&$  3890 $&$ ^{+280}_{-280} $&$  0.43 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -86.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.70 $ \\
$1000575$&$  266.32120 $&$   -29.130648 $&$  3570 $&$ ^{+300}_{-320} $&$  0.30 $&$ ^{+0.35}_{-0.38} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -75.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.83 $ \\
$1000576$&$  266.32611 $&$   -29.126017 $&$  3780 $&$ ^{+310}_{-300} $&$  0.72 $&$ ^{+0.36}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$     21.6 $&$ ^{+ 3.2}_{- 3.2} $&$  12.90 $ \\
$1000634$&$  266.33145 $&$   -29.137831 $&$  3300 $&$ ^{+280}_{-280} $&$  0.80 $&$ ^{+0.35}_{-0.35} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     74.6 $&$ ^{+ 3.1}_{- 3.1} $&$   9.24 $ \\
$1000636$&$  266.32977 $&$   -29.140060 $&$  3840 $&$ ^{+290}_{-290} $&$  0.11 $&$ ^{+0.42}_{-0.42} $&$  0.6 $&$ ^{+1.3}_{-1.3} $&$     45.6 $&$ ^{+ 2.1}_{- 2.1} $&$  10.20 $ \\
$1000761$&$  266.32782 $&$   -29.141058 $&$  3900 $&$ ^{+280}_{-280} $&$  0.01 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -33.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.17 $ \\
$1000773$&$  266.32852 $&$   -29.140715 $&$  3410 $&$ ^{+280}_{-280} $&$  0.58 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -54.6 $&$ ^{+ 3.1}_{- 3.1} $&$  10.99 $ \\
$1000777$&$  266.33179 $&$   -29.137058 $&$  4120 $&$ ^{+280}_{-280} $&$ -0.30 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -23.9 $&$ ^{+ 3.1}_{- 3.1} $&$  11.89 $ \\
$1001528$&$  266.33502 $&$   -29.129675 $&$  3500 $&$ ^{+310}_{-310} $&$  0.48 $&$ ^{+0.33}_{-0.33} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$     -1.9 $&$ ^{+ 0.6}_{- 0.6} $&$  10.46 $ \\
$1001529$&$  266.32617 $&$   -29.141619 $&$  3910 $&$ ^{+280}_{-280} $&$ -0.06 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -50.6 $&$ ^{+ 3.1}_{- 3.1} $&$  10.75 $ \\
$1001532$&$  266.33182 $&$   -29.136072 $&$  3460 $&$ ^{+270}_{-270} $&$  0.47 $&$ ^{+0.40}_{-0.40} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -140.1 $&$ ^{+ 0.7}_{- 0.7} $&$  11.57 $ \\
$1001539$&$  266.32993 $&$   -29.136271 $&$  3940 $&$ ^{+280}_{-280} $&$ -0.07 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -52.4 $&$ ^{+ 1.5}_{- 1.5} $&$  11.78 $ \\
$1001542$&$  266.33392 $&$   -29.129133 $&$  3810 $&$ ^{+280}_{-280} $&$  0.09 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     46.2 $&$ ^{+ 4.7}_{- 4.7} $&$  11.86 $ \\
$1001543$&$  266.32950 $&$   -29.138340 $&$  3920 $&$ ^{+280}_{-270} $&$  0.93 $&$ ^{+0.32}_{-0.32} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -20.3 $&$ ^{+ 1.3}_{- 1.3} $&$  12.49 $ \\
$1001544$&$  266.33774 $&$   -29.127413 $&$  3450 $&$ ^{+280}_{-280} $&$  0.82 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -26.6 $&$ ^{+ 2.5}_{- 2.5} $&$  11.40 $ \\
$1001545$&$  266.32751 $&$   -29.138519 $&$  3760 $&$ ^{+320}_{-320} $&$  0.73 $&$ ^{+0.43}_{-0.43} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -82.7 $&$ ^{+ 1.3}_{- 1.3} $&$  11.87 $ \\
$1001546$&$  266.33160 $&$   -29.132668 $&$  3700 $&$ ^{+300}_{-310} $&$  0.35 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$   -122.4 $&$ ^{+ 3.1}_{- 3.1} $&$  11.88 $ \\
$1001548$&$  266.33224 $&$   -29.135014 $&$  4070 $&$ ^{+280}_{-280} $&$ -0.04 $&$ ^{+0.35}_{-0.35} $&$  2.8 $&$ ^{+1.1}_{-1.2} $&$    -94.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.29 $ \\
$1001549$&$  266.33301 $&$   -29.133286 $&$  3960 $&$ ^{+280}_{-280} $&$  0.59 $&$ ^{+0.34}_{-0.38} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -81.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.40 $ \\
$1001554$&$  266.32846 $&$   -29.138165 $&$  3860 $&$ ^{+300}_{-300} $&$  0.92 $&$ ^{+0.32}_{-0.32} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$   -126.7 $&$ ^{+ 5.8}_{- 5.8} $&$  12.16 $ \\
$1001564$&$  266.32727 $&$   -29.139542 $&$  4040 $&$ ^{+280}_{-280} $&$  0.33 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -63.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.47 $ \\
$1001568$&$  266.33463 $&$   -29.131060 $&$  4260 $&$ ^{+290}_{-300} $&$ -0.32 $&$ ^{+0.35}_{-0.35} $&$  3.6 $&$ ^{+1.1}_{-1.1} $&$     60.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.34 $ \\
$1001574$&$  266.33578 $&$   -29.126301 $&$  3980 $&$ ^{+280}_{-280} $&$ -0.15 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -24.6 $&$ ^{+ 2.6}_{- 2.6} $&$  11.89 $ \\
$1001589$&$  266.33035 $&$   -29.134398 $&$  4150 $&$ ^{+290}_{-300} $&$  0.67 $&$ ^{+0.35}_{-0.35} $&$  3.7 $&$ ^{+1.1}_{-1.1} $&$    -34.8 $&$ ^{+ 4.1}_{- 4.3} $&$  13.20 $ \\
$1001590$&$  266.33606 $&$   -29.128407 $&$  3970 $&$ ^{+300}_{-310} $&$  0.58 $&$ ^{+0.35}_{-0.36} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$    -47.4 $&$ ^{+ 3.1}_{- 3.1} $&$  13.09 $ \\
$1001603$&$  266.32635 $&$   -29.140284 $&$  3790 $&$ ^{+290}_{-290} $&$  0.87 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -84.8 $&$ ^{+ 3.1}_{- 3.1} $&$  12.25 $ \\
$1001628$&$  266.32541 $&$   -29.127810 $&$  3900 $&$ ^{+280}_{-280} $&$ -0.71 $&$ ^{+0.35}_{-0.35} $&$  1.1 $&$ ^{+1.1}_{-1.0} $&$    153.3 $&$ ^{+ 3.1}_{- 3.1} $&$  10.99 $ \\
$1001630$&$  266.33347 $&$   -29.124790 $&$  3740 $&$ ^{+280}_{-280} $&$  0.05 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    106.8 $&$ ^{+ 3.1}_{- 3.1} $&$  10.77 $ \\
$1001631$&$  266.32159 $&$   -29.136383 $&$  3520 $&$ ^{+290}_{-290} $&$  0.14 $&$ ^{+0.37}_{-0.37} $&$  0.0 $&$ ^{+1.0}_{-1.0} $&$    -20.0 $&$ ^{+ 4.7}_{- 4.7} $&$  10.13 $ \\
$1001633$&$  266.33170 $&$   -29.124191 $&$  4190 $&$ ^{+290}_{-280} $&$ -0.48 $&$ ^{+0.35}_{-0.35} $&$  3.9 $&$ ^{+1.0}_{-1.0} $&$     46.2 $&$ ^{+ 3.1}_{- 3.1} $&$  11.08 $ \\
$1001635$&$  266.32578 $&$   -29.123371 $&$  3600 $&$ ^{+280}_{-280} $&$  0.14 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    126.4 $&$ ^{+ 3.1}_{- 3.1} $&$  10.87 $ \\
$1001636$&$  266.33456 $&$   -29.126963 $&$  3590 $&$ ^{+280}_{-280} $&$  0.46 $&$ ^{+0.35}_{-0.35} $&$  0.9 $&$ ^{+1.0}_{-1.0} $&$    -15.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.10 $ \\
$1001639$&$  266.32043 $&$   -29.139029 $&$  3880 $&$ ^{+280}_{-280} $&$ -0.31 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -55.9 $&$ ^{+ 3.1}_{- 3.1} $&$  11.19 $ \\
$1001640$&$  266.32355 $&$   -29.134727 $&$  4120 $&$ ^{+280}_{-280} $&$ -0.36 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -76.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.36 $ \\
$1001641$&$  266.33160 $&$   -29.131948 $&$  3940 $&$ ^{+280}_{-280} $&$ -0.23 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    105.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.75 $ \\
$1001643$&$  266.32941 $&$   -29.131618 $&$  3690 $&$ ^{+280}_{-280} $&$  0.17 $&$ ^{+0.35}_{-0.35} $&$  0.4 $&$ ^{+1.0}_{-1.0} $&$    -51.0 $&$ ^{+ 3.1}_{- 3.1} $&$  10.90 $ \\
$1001649$&$  266.32001 $&$   -29.137936 $&$  4170 $&$ ^{+290}_{-290} $&$ -0.14 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -79.9 $&$ ^{+ 2.8}_{- 2.8} $&$  11.52 $ \\
$1001652$&$  266.32446 $&$   -29.137747 $&$  3500 $&$ ^{+290}_{-290} $&$  0.72 $&$ ^{+0.32}_{-0.32} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -96.4 $&$ ^{+ 2.4}_{- 2.4} $&$  11.37 $ \\
$1001653$&$  266.33142 $&$   -29.128298 $&$  3840 $&$ ^{+280}_{-280} $&$ -0.10 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     75.1 $&$ ^{+ 0.8}_{- 0.8} $&$  11.42 $ \\
$1001654$&$  266.32675 $&$   -29.134991 $&$  4160 $&$ ^{+280}_{-280} $&$ -0.13 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -48.4 $&$ ^{+ 3.1}_{- 3.1} $&$  11.78 $ \\
$1001657$&$  266.31827 $&$   -29.133718 $&$  3890 $&$ ^{+270}_{-270} $&$  0.10 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     13.0 $&$ ^{+ 3.7}_{- 3.7} $&$  11.49 $ \\
$1001658$&$  266.32773 $&$   -29.122234 $&$  3870 $&$ ^{+280}_{-280} $&$ -0.30 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     44.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.51 $ \\
$1001659$&$  266.32245 $&$   -29.135933 $&$  3880 $&$ ^{+270}_{-270} $&$  0.15 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$   -107.0 $&$ ^{+ 1.7}_{- 1.7} $&$  11.61 $ \\
$1001660$&$  266.32132 $&$   -29.137897 $&$  3420 $&$ ^{+320}_{-320} $&$  0.81 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -95.1 $&$ ^{+ 2.3}_{- 2.3} $&$  11.61 $ \\
$1001665$&$  266.32480 $&$   -29.138943 $&$  4380 $&$ ^{+320}_{-320} $&$  0.17 $&$ ^{+0.35}_{-0.35} $&$  3.3 $&$ ^{+1.2}_{-1.2} $&$    -63.6 $&$ ^{+ 4.6}_{- 4.6} $&$  11.65 $ \\
$1001667$&$  266.32205 $&$   -29.137917 $&$  4090 $&$ ^{+270}_{-270} $&$ -0.06 $&$ ^{+0.36}_{-0.36} $&$  0.6 $&$ ^{+1.3}_{-1.3} $&$    -47.6 $&$ ^{+ 1.5}_{- 1.5} $&$  11.68 $ \\
$1001668$&$  266.32779 $&$   -29.133268 $&$  4100 $&$ ^{+280}_{-290} $&$  0.01 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$     51.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.94 $ \\
$1001671$&$  266.32773 $&$   -29.132935 $&$  3800 $&$ ^{+290}_{-270} $&$  0.25 $&$ ^{+0.33}_{-0.33} $&$  0.4 $&$ ^{+1.0}_{-1.0} $&$     -7.4 $&$ ^{+ 2.5}_{- 2.5} $&$  11.82 $ \\
$1001674$&$  266.32056 $&$   -29.131559 $&$  3910 $&$ ^{+280}_{-270} $&$ -0.32 $&$ ^{+0.32}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     83.8 $&$ ^{+ 2.9}_{- 2.9} $&$  11.45 $ \\
$1001675$&$  266.32883 $&$   -29.130363 $&$  3780 $&$ ^{+280}_{-280} $&$  0.17 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    175.0 $&$ ^{+ 3.1}_{- 3.1} $&$  11.60 $ \\
$1001676$&$  266.33206 $&$   -29.130527 $&$  3880 $&$ ^{+280}_{-280} $&$  0.51 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$   -203.2 $&$ ^{+ 3.1}_{- 3.1} $&$  12.10 $ \\
$1001679$&$  266.33334 $&$   -29.126389 $&$  3870 $&$ ^{+290}_{-270} $&$  0.16 $&$ ^{+0.33}_{-0.33} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -20.4 $&$ ^{+ 4.9}_{- 4.9} $&$  11.76 $ \\
$1001683$&$  266.32230 $&$   -29.132397 $&$  3870 $&$ ^{+280}_{-280} $&$  0.19 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -25.8 $&$ ^{+ 3.1}_{- 3.1} $&$  11.86 $ \\
$1001684$&$  266.32617 $&$   -29.121529 $&$  3690 $&$ ^{+280}_{-280} $&$  0.63 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -55.9 $&$ ^{+ 3.1}_{- 3.1} $&$  11.76 $ \\
$1001687$&$  266.33127 $&$   -29.130116 $&$  4340 $&$ ^{+640}_{-640} $&$  0.49 $&$ ^{+0.33}_{-0.33} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$   -112.0 $&$ ^{+ 1.5}_{- 1.5} $&$  12.17 $ \\
$1001689$&$  266.32748 $&$   -29.135292 $&$  4240 $&$ ^{+310}_{-310} $&$ -0.07 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -94.0 $&$ ^{+ 1.9}_{- 1.9} $&$  12.03 $ \\
$1001690$&$  266.32260 $&$   -29.127846 $&$  3600 $&$ ^{+310}_{-310} $&$  0.61 $&$ ^{+0.38}_{-0.38} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -20.4 $&$ ^{+ 1.7}_{- 1.7} $&$  11.46 $ \\
$1001695$&$  266.33093 $&$   -29.130344 $&$  3990 $&$ ^{+400}_{-400} $&$  0.55 $&$ ^{+0.37}_{-0.37} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     44.1 $&$ ^{+ 4.6}_{- 4.6} $&$  12.11 $ \\
$1001703$&$  266.32080 $&$   -29.137960 $&$  4100 $&$ ^{+300}_{-290} $&$ -0.88 $&$ ^{+0.38}_{-0.36} $&$  3.0 $&$ ^{+1.4}_{-1.2} $&$    212.2 $&$ ^{+ 3.1}_{- 3.1} $&$  11.94 $ \\
$1001704$&$  266.31934 $&$   -29.132509 $&$  3850 $&$ ^{+280}_{-280} $&$  0.01 $&$ ^{+0.34}_{-0.34} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -11.7 $&$ ^{+ 2.2}_{- 2.2} $&$  11.88 $ \\
$1001709$&$  266.32199 $&$   -29.138540 $&$  4250 $&$ ^{+290}_{-290} $&$  0.11 $&$ ^{+0.33}_{-0.33} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -85.5 $&$ ^{+ 9.5}_{- 9.5} $&$  12.16 $ \\
$1001713$&$  266.32321 $&$   -29.135204 $&$  4730 $&$ ^{+310}_{-290} $&$  0.23 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$    -70.5 $&$ ^{+ 3.1}_{- 3.1} $&$  12.03 $ \\
$1001716$&$  266.33353 $&$   -29.132507 $&$  3930 $&$ ^{+280}_{-280} $&$  0.35 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -27.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.33 $ \\
$1001721$&$  266.33231 $&$   -29.129238 $&$  4150 $&$ ^{+280}_{-280} $&$  0.57 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$   -159.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.21 $ \\
$1001722$&$  266.32812 $&$   -29.135983 $&$  4190 $&$ ^{+290}_{-280} $&$  0.58 $&$ ^{+0.35}_{-0.35} $&$  2.9 $&$ ^{+1.0}_{-1.0} $&$    -91.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.27 $ \\
$1001727$&$  266.32996 $&$   -29.131516 $&$  3860 $&$ ^{+280}_{-280} $&$  0.89 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -52.1 $&$ ^{+ 3.1}_{- 3.1} $&$  12.12 $ \\
$1001735$&$  266.32141 $&$   -29.134857 $&$  3880 $&$ ^{+280}_{-280} $&$  0.17 $&$ ^{+0.35}_{-0.35} $&$  0.3 $&$ ^{+1.0}_{-1.0} $&$     31.1 $&$ ^{+ 3.1}_{- 3.1} $&$  11.80 $ \\
$1001737$&$  266.32443 $&$   -29.136889 $&$  4340 $&$ ^{+330}_{-320} $&$  0.05 $&$ ^{+0.37}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.2} $&$   -198.1 $&$ ^{+ 7.0}_{- 6.7} $&$  12.43 $ \\
$1001745$&$  266.33109 $&$   -29.124212 $&$  3860 $&$ ^{+280}_{-270} $&$  0.18 $&$ ^{+0.38}_{-0.38} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$     60.6 $&$ ^{+ 1.0}_{- 0.9} $&$  11.97 $ \\
$1001746$&$  266.33160 $&$   -29.124517 $&$  3810 $&$ ^{+300}_{-300} $&$  0.71 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$   -138.6 $&$ ^{+ 3.1}_{- 3.1} $&$  12.10 $ \\
$1001749$&$  266.32098 $&$   -29.138306 $&$  4120 $&$ ^{+290}_{-290} $&$  0.67 $&$ ^{+0.35}_{-0.35} $&$  3.1 $&$ ^{+1.1}_{-1.1} $&$    -39.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.23 $ \\
$1001750$&$  266.32376 $&$   -29.137165 $&$  4090 $&$ ^{+300}_{-290} $&$  0.02 $&$ ^{+0.35}_{-0.35} $&$  0.6 $&$ ^{+1.0}_{-1.1} $&$    -26.4 $&$ ^{+ 7.8}_{- 7.8} $&$  11.73 $ \\
$1001751$&$  266.33127 $&$   -29.128775 $&$  4090 $&$ ^{+290}_{-290} $&$  0.10 $&$ ^{+0.36}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -12.6 $&$ ^{+ 3.6}_{- 3.1} $&$  12.46 $ \\
$1001758$&$  266.32605 $&$   -29.124632 $&$  4190 $&$ ^{+310}_{-320} $&$ -0.55 $&$ ^{+0.37}_{-0.37} $&$  3.4 $&$ ^{+1.3}_{-1.2} $&$      5.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.24 $ \\
$1001761$&$  266.32877 $&$   -29.129723 $&$  4320 $&$ ^{+310}_{-300} $&$  0.31 $&$ ^{+0.34}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     30.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.55 $ \\
$1001767$&$  266.32761 $&$   -29.131617 $&$  4360 $&$ ^{+320}_{-300} $&$  0.29 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -96.6 $&$ ^{+ 3.4}_{- 3.5} $&$  12.22 $ \\
$1001771$&$  266.32709 $&$   -29.131716 $&$  4120 $&$ ^{+340}_{-340} $&$  0.37 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -26.7 $&$ ^{+ 1.4}_{- 1.4} $&$  12.15 $ \\
$1001779$&$  266.32504 $&$   -29.136560 $&$  3960 $&$ ^{+280}_{-280} $&$ -0.04 $&$ ^{+0.33}_{-0.33} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -58.9 $&$ ^{+ 1.0}_{- 1.0} $&$  11.95 $ \\
$1001784$&$  266.33389 $&$   -29.125143 $&$  4130 $&$ ^{+300}_{-300} $&$ -0.15 $&$ ^{+0.36}_{-0.37} $&$  4.1 $&$ ^{+1.2}_{-1.1} $&$     91.3 $&$ ^{+ 3.1}_{- 3.1} $&$  12.17 $ \\
$1001786$&$  266.32550 $&$   -29.138453 $&$  3920 $&$ ^{+280}_{-290} $&$  0.51 $&$ ^{+0.38}_{-0.38} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     -9.1 $&$ ^{+ 2.8}_{- 2.8} $&$  12.43 $ \\
$1001790$&$  266.32333 $&$   -29.133156 $&$  4630 $&$ ^{+300}_{-320} $&$  0.35 $&$ ^{+0.35}_{-0.35} $&$  2.7 $&$ ^{+1.1}_{-1.3} $&$    -89.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.26 $ \\
$1001793$&$  266.32315 $&$   -29.136534 $&$  3930 $&$ ^{+280}_{-280} $&$ -0.05 $&$ ^{+0.39}_{-0.39} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -40.7 $&$ ^{+ 1.9}_{- 1.9} $&$  11.94 $ \\
$1001813$&$  266.33344 $&$   -29.126656 $&$  3900 $&$ ^{+280}_{-280} $&$ -0.11 $&$ ^{+0.35}_{-0.39} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -61.9 $&$ ^{+ 4.1}_{- 3.5} $&$  12.31 $ \\
$1001816$&$  266.32135 $&$   -29.139233 $&$  4170 $&$ ^{+300}_{-300} $&$ -0.01 $&$ ^{+0.36}_{-0.35} $&$  3.3 $&$ ^{+1.3}_{-1.3} $&$    -48.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.52 $ \\
$1001838$&$  266.32150 $&$   -29.138630 $&$  3810 $&$ ^{+290}_{-290} $&$  0.93 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     -0.3 $&$ ^{+ 3.1}_{- 3.1} $&$  12.46 $ \\
$1001848$&$  266.32593 $&$   -29.128468 $&$  4030 $&$ ^{+310}_{-320} $&$  0.54 $&$ ^{+0.35}_{-0.36} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -93.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.84 $ \\
$1001853$&$  266.32846 $&$   -29.128000 $&$  4100 $&$ ^{+280}_{-280} $&$  0.28 $&$ ^{+0.33}_{-0.33} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$     23.8 $&$ ^{+ 3.9}_{- 3.9} $&$  12.64 $ \\
$1001858$&$  266.32922 $&$   -29.135126 $&$  3900 $&$ ^{+290}_{-290} $&$  0.73 $&$ ^{+0.41}_{-0.41} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -30.7 $&$ ^{+ 1.3}_{- 1.2} $&$  12.17 $ \\
$1001859$&$  266.32812 $&$   -29.124929 $&$  4200 $&$ ^{+340}_{-340} $&$  0.07 $&$ ^{+0.36}_{-0.36} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$    -27.6 $&$ ^{+ 5.7}_{- 5.7} $&$  12.45 $ \\
$1001875$&$  266.33301 $&$   -29.127167 $&$  3850 $&$ ^{+320}_{-320} $&$  0.36 $&$ ^{+0.38}_{-0.38} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$   -142.6 $&$ ^{+ 2.6}_{- 2.6} $&$  12.59 $ \\
$1001885$&$  266.32135 $&$   -29.136299 $&$  3910 $&$ ^{+280}_{-280} $&$  0.65 $&$ ^{+0.38}_{-0.38} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -41.9 $&$ ^{+ 2.8}_{- 2.8} $&$  12.49 $ \\
$1001889$&$  266.32251 $&$   -29.131845 $&$  3870 $&$ ^{+280}_{-280} $&$  0.29 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -29.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.20 $ \\
$1001911$&$  266.32635 $&$   -29.136511 $&$  4320 $&$ ^{+290}_{-300} $&$ -0.41 $&$ ^{+0.35}_{-0.35} $&$  3.3 $&$ ^{+1.2}_{-1.1} $&$   -333.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.39 $ \\
$1001927$&$  266.32269 $&$   -29.127436 $&$  4060 $&$ ^{+280}_{-280} $&$  0.34 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -12.6 $&$ ^{+ 3.1}_{- 3.1} $&$  12.73 $ \\
$1001929$&$  266.33591 $&$   -29.125961 $&$  3930 $&$ ^{+280}_{-280} $&$  0.79 $&$ ^{+0.35}_{-0.34} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -19.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.06 $ \\
$1001930$&$  266.32315 $&$   -29.128483 $&$  4510 $&$ ^{+350}_{-330} $&$ -1.21 $&$ ^{+0.37}_{-0.38} $&$  3.7 $&$ ^{+1.3}_{-1.1} $&$    159.7 $&$ ^{+ 6.1}_{- 6.0} $&$  12.11 $ \\
$1001947$&$  266.32996 $&$   -29.126337 $&$  3960 $&$ ^{+280}_{-280} $&$  0.50 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$     -5.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.63 $ \\
$1001948$&$  266.32562 $&$   -29.134995 $&$  4490 $&$ ^{+330}_{-300} $&$  0.04 $&$ ^{+0.35}_{-0.35} $&$  4.1 $&$ ^{+1.2}_{-1.0} $&$    -59.2 $&$ ^{+ 4.6}_{- 5.0} $&$  12.84 $ \\
$1001970$&$  266.32822 $&$   -29.136164 $&$  4360 $&$ ^{+300}_{-290} $&$  0.11 $&$ ^{+0.37}_{-0.35} $&$  2.9 $&$ ^{+1.1}_{-1.1} $&$    -33.9 $&$ ^{+ 6.4}_{- 6.7} $&$  13.13 $ \\
$1001992$&$  266.32590 $&$   -29.130253 $&$  4380 $&$ ^{+300}_{-310} $&$  0.52 $&$ ^{+0.35}_{-0.35} $&$  3.0 $&$ ^{+1.1}_{-1.1} $&$     21.4 $&$ ^{+ 3.1}_{- 3.1} $&$  12.91 $ \\
$1002027$&$  266.32635 $&$   -29.132494 $&$  4000 $&$ ^{+280}_{-280} $&$  0.56 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$      7.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.44 $ \\
$1002035$&$  266.32385 $&$   -29.137501 $&$  4120 $&$ ^{+280}_{-300} $&$  0.52 $&$ ^{+0.35}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.1} $&$    -46.0 $&$ ^{+ 3.1}_{- 3.1} $&$  12.81 $ \\
$1002042$&$  266.32858 $&$   -29.132753 $&$  4020 $&$ ^{+280}_{-280} $&$  0.51 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -63.1 $&$ ^{+ 3.1}_{- 3.1} $&$  12.29 $ \\
$1002112$&$  266.31927 $&$   -29.137617 $&$  3920 $&$ ^{+280}_{-280} $&$  0.51 $&$ ^{+0.35}_{-0.37} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$   -112.9 $&$ ^{+ 3.1}_{- 3.1} $&$  12.62 $ \\
$1002122$&$  266.31888 $&$   -29.136415 $&$  3920 $&$ ^{+280}_{-280} $&$  0.85 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$     21.7 $&$ ^{+ 3.1}_{- 3.1} $&$  12.68 $ \\
$1002225$&$  266.32339 $&$   -29.135481 $&$  4200 $&$ ^{+360}_{-360} $&$  0.54 $&$ ^{+0.40}_{-0.40} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$    -66.0 $&$ ^{+ 1.7}_{- 1.6} $&$  12.74 $ \\
$1002230$&$  266.32834 $&$   -29.134781 $&$  4240 $&$ ^{+290}_{-280} $&$  0.44 $&$ ^{+0.35}_{-0.35} $&$  4.4 $&$ ^{+1.0}_{-1.0} $&$    -47.6 $&$ ^{+ 3.1}_{- 3.1} $&$  13.14 $ \\
$1002297$&$  266.32721 $&$   -29.125605 $&$  4370 $&$ ^{+310}_{-310} $&$ -0.10 $&$ ^{+0.39}_{-0.39} $&$  2.7 $&$ ^{+1.1}_{-1.2} $&$   -143.5 $&$ ^{+ 6.4}_{- 7.0} $&$  13.22 $ \\
$1002349$&$  266.32092 $&$   -29.130215 $&$  3930 $&$ ^{+280}_{-280} $&$  0.36 $&$ ^{+0.35}_{-0.35} $&$  2.1 $&$ ^{+1.0}_{-1.0} $&$    -74.9 $&$ ^{+ 3.1}_{- 3.1} $&$  13.06 $ \\
$1002373$&$  266.31927 $&$   -29.135080 $&$  4180 $&$ ^{+300}_{-330} $&$  0.17 $&$ ^{+0.34}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.1} $&$    -85.9 $&$ ^{+ 5.0}_{- 5.0} $&$  13.09 $ \\
$1002455$&$  266.31909 $&$   -29.137529 $&$  4440 $&$ ^{+280}_{-290} $&$ -0.08 $&$ ^{+0.35}_{-0.35} $&$  2.4 $&$ ^{+1.0}_{-1.2} $&$    -62.8 $&$ ^{+ 6.5}_{- 6.0} $&$  13.05 $ \\
$1002511$&$  266.32693 $&$   -29.137909 $&$  4340 $&$ ^{+320}_{-310} $&$  0.10 $&$ ^{+0.36}_{-0.36} $&$  2.6 $&$ ^{+1.1}_{-1.1} $&$    -72.5 $&$ ^{+ 4.9}_{- 4.6} $&$  13.33 $ \\
$1002546$&$  266.32428 $&$   -29.131695 $&$  4130 $&$ ^{+300}_{-330} $&$  0.81 $&$ ^{+0.35}_{-0.34} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$     54.6 $&$ ^{+ 3.1}_{- 3.1} $&$  12.85 $ \\
$1002567$&$  266.32077 $&$   -29.134623 $&$  3740 $&$ ^{+290}_{-290} $&$  0.90 $&$ ^{+0.35}_{-0.35} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -27.8 $&$ ^{+ 3.1}_{- 3.1} $&$  13.09 $ \\
$1002642$&$  266.32071 $&$   -29.130146 $&$  4070 $&$ ^{+300}_{-310} $&$  0.26 $&$ ^{+0.40}_{-0.36} $&$  2.8 $&$ ^{+1.1}_{-1.2} $&$    -83.7 $&$ ^{+ 6.8}_{- 6.4} $&$  13.49 $ \\
$1003321$&$  266.33359 $&$   -29.134296 $&$  3400 $&$ ^{+270}_{-270} $&$  0.62 $&$ ^{+0.37}_{-0.37} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$      6.2 $&$ ^{+10.8}_{-10.8} $&$  11.39 $ \\
$1003333$&$  266.33652 $&$   -29.130331 $&$  3890 $&$ ^{+280}_{-280} $&$ -0.21 $&$ ^{+0.35}_{-0.35} $&$  0.2 $&$ ^{+1.0}_{-1.0} $&$    -13.7 $&$ ^{+ 3.1}_{- 3.1} $&$  11.86 $ \\
$1003344$&$  266.33554 $&$   -29.131725 $&$  3540 $&$ ^{+280}_{-280} $&$ -0.14 $&$ ^{+0.35}_{-0.35} $&$  0.1 $&$ ^{+1.0}_{-1.0} $&$    -77.3 $&$ ^{+ 3.1}_{- 3.1} $&$  11.88 $ \\
$1003372$&$  266.33078 $&$   -29.138859 $&$  4070 $&$ ^{+280}_{-300} $&$  0.37 $&$ ^{+0.35}_{-0.34} $&$  2.5 $&$ ^{+1.1}_{-1.1} $&$     85.2 $&$ ^{+ 3.3}_{- 3.2} $&$  12.83 $ \\
$1003393$&$  266.32947 $&$   -29.139988 $&$  3990 $&$ ^{+280}_{-280} $&$  0.37 $&$ ^{+0.35}_{-0.35} $&$  2.3 $&$ ^{+1.0}_{-1.1} $&$   -135.2 $&$ ^{+ 3.5}_{- 3.6} $&$  12.55 $ \\
$1003498$&$  266.33127 $&$   -29.135870 $&$  3980 $&$ ^{+290}_{-290} $&$  0.54 $&$ ^{+0.33}_{-0.34} $&$  2.2 $&$ ^{+1.0}_{-1.0} $&$    -97.1 $&$ ^{+ 3.7}_{- 3.7} $&$  12.76 $ \\
$1003681$&$  266.33380 $&$   -29.134117 $&$  4180 $&$ ^{+300}_{-310} $&$ -0.20 $&$ ^{+0.36}_{-0.38} $&$  2.3 $&$ ^{+1.0}_{-1.0} $&$      9.2 $&$ ^{+ 6.2}_{- 7.1} $&$  13.45 $ \\
\hline
\end{tabular}
\end{table}

